Instance-dependent Noisy-label Learning with Graphical Model Based Noise-rate Estimation

Deep learning faces a formidable challenge when handling noisy labels, as models tend to overfit samples affected by label noise. This challenge is further compounded by the presence of instance-dependent noise (IDN), a realistic form of label noise arising from ambiguous sample information. To address IDN, Label Noise Learning (LNL) incorporates a sample selection stage to differentiate clean and noisy-label samples. This stage uses an arbitrary criterion and a pre-defined curriculum that initially selects most samples as noisy and gradually decreases this selection rate during training. Such curriculum is sub-optimal since it does not consider the actual label noise rate in the training set. This paper addresses this issue with a new noise-rate estimation method that is easily integrated with most state-of-the-art (SOTA) LNL methods to produce a more effective curriculum. Synthetic and real-world benchmark results demonstrate that integrating our approach with SOTA LNL methods improves accuracy in most cases.

==> csvs/ablation_table.tex <==
\begin{table}[ht]
        \centering
        \caption{\emph{(left)} Ablation results showing the test accuracy \% on CIFAR100~\cite{krizhevsky2009learning} at \(0.5\) IDN~\cite{xia2020part}. First, we display the results of base DivideMix~\cite{li2020dividemix}, followed by the ideal case (result in \textit{italics}), where we assume to know the correct \(\epsilon=50\%\) for the sample selection before training. In the third case, we incorporate a pre-trained DivideMix~\cite{li2020dividemix} into our model, whilst the next case shows our proposed model and  DivideMix~\cite{li2020dividemix} being trained together, but using DivideMix's~\cite{li2020dividemix} sample selection curriculum, not our estimated \(\epsilon\). The last row shows the results of our proposed complete model with DivideMix~\cite{li2020dividemix}. \emph{(right)} This table shows the training time of the base model DivideMix~\cite{li2020dividemix} and our approach with DivideMix~\cite{li2020dividemix} at \(0.5\) IDN~\cite{xia2020part} on the mentioned computational settings~\cref{subsec:implementation}. }
        \label{tab:ablation_cifar}
        % \resizebox{0.4\textwidth}{!} {
        \begin{subtable}[t]{.45\linewidth}
        \addtolength{\tabcolsep}{-0.1em}
        \centering
        \begin{tabular}{l c}
            \toprule
            \bfseries Models &  \bfseries Test Accuracy (\%) \\
            \midrule
            DivideMix & 58.61 \\
            DivideMix with fix \(\epsilon\) (ideal case) & 64.44 \\
            Proposed with pre-trained DivideMix &  52.31\\
            Proposed with original DivideMix (no \(\epsilon\)) & 56.30\\
            \rowcolor{Gray!25} \textbf{DivideMix-Ours} & \textbf{64.02} \\
            \bottomrule
        \end{tabular}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{.3\linewidth}
        \centering
        \addtolength{\tabcolsep}{-0.4em}
        \begin{tabular}{c c}
        \toprule
        \textbf{Model} & \textbf{Time (hrs)} \\
        \midrule
        DivideMix~\cite{li2020dividemix} & \(7.2\) \\
        DivideMix-Ours & \(13.1\) \\
        \bottomrule
        \end{tabular}
        \end{subtable}        
\end{table}

% \begin{table}[htbp!]
%         \caption{This table shows the training time of the base model DivideMix~\cite{li2020dividemix} and our approach with DivideMix~\cite{li2020dividemix} at \(0.5\) IDN~\cite{xia2020part} on the mentioned computational settings~\cref{subsec:implementation}.}
%         \label{table:computation}
%         \centering
%         \begin{tabular}{c c}
%         \toprule
%         \textbf{Model} & \textbf{Time (hrs)} \\
%         \midrule
%         DivideMix~\cite{li2020dividemix} & \(7.2\) \\
%         DivideMix-Ours & \(12.1\) \\
%         \bottomrule
%         \end{tabular}
% \end{table}

==> csvs/cifar_table.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Test accuracy \% on CIFAR100~\cite{krizhevsky2009learning} under different IDN~\cite{xiao2015learning}. Other models results are presented in~\cite{garg2023instance,cheng2022instance}. Here, we use DivideMix~\cite{li2020dividemix} and InstanceGM~\cite{garg2023instance} as the baselines for our proposed work. Estimated noise rates \(\epsilon\) are also highlighted in the table. }
%     \begin{minipage}{.45\linewidth}
%     \centering
%     \begin{subtable}{\linewidth}
%     \begin{tabular}{l l l l l}
%     \toprule
%     \multirow{2}{*}{\bfseries Method } & \multicolumn{4}{c}{\bfseries Noise Rates - IDN} \\
%     \cmidrule{2 - 5} 
%     & \textbf{0.2} & \textbf{0.3} & \textbf{0.4} & \textbf{0.5} \\
%     \midrule
%     CE~\cite{yao2021instance} & 30.42 & 24.15 & 21.45 & 14.42 \\
%     PartT~\cite{xia2020part} & 65.33 & 64.56 & 59.73 & 56.80\\
%     kMEIDTM~\cite{cheng2022instance} & 69.16 & 66.76 & 63.46 & 59.18\\
%     \midrule
%     DivideMix~\cite{li2020dividemix} & 77.03 & 76.33 & 70.80 & 58.61\\
%     \rowcolor{Gray!25}\textbf{DivideMix-Ours} & \textbf{77.42} & \textbf{77.21} & \textbf{72.41} & \textbf{64.02}\\
%     % \hdashline
%     \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.18}} & \scriptsize{\textbf{0.34}} & \scriptsize{\textbf{0.47}} & \scriptsize{\textbf{0.53}}\\
%     \midrule
%     InstanceGM~\cite{garg2023instance} & \textbf{79.69} & 79.21 & 78.47 & 77.19\\
%     \rowcolor{Gray!25} \textbf{InstanceGM-Ours} & 79.61 & \textbf{79.40} & \textbf{79.52} & \textbf{77.76}\\
%     % \hdashline
%     \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.32}} & \scriptsize{\textbf{0.37}} & \scriptsize{\textbf{0.42}} & \scriptsize{\textbf{0.47}}\\
%     % \bottomrule
%     \end{tabular}
%     \end{subtable}
%     \end{minipage}
% \end{table}
\begin{table}[t]
    \centering
    \caption{\emph{(left)} Test accuracy \% and \emph{(right)} final estimated noise rate \(\epsilon\) on CIFAR100~\cite{krizhevsky2009learning} under different IDN~\cite{xiao2015learning}. Other models' results are from~\cite{garg2023instance,cheng2022instance}. Here, we integrate DivideMix~\cite{li2020dividemix} and InstanceGM~\cite{garg2023instance} into our proposed model.}
    \label{table:cifar100}
    \begin{subtable}[t]{0.35\linewidth}
        \centering
        \addtolength{\tabcolsep}{-0.1em}
        \begin{tabular}{l c c c c}
            \toprule
            \multirow{2}{*}{\bfseries Method } & \multicolumn{4}{c}{\bfseries Noise Rates - IDN} \\
            \cmidrule{2 - 5} 
            & \textbf{0.2} & \textbf{0.3} & \textbf{0.4} & \textbf{0.5} \\
            \midrule
            CE~\cite{yao2021instance} & 30.42 & 24.15 & 21.45 & 14.42 \\
            PartT~\cite{xia2020part} & 65.33 & 64.56 & 59.73 & 56.80\\
            kMEIDTM~\cite{cheng2022instance} & 69.16 & 66.76 & 63.46 & 59.18\\
            \midrule
            DivideMix~\cite{li2020dividemix} & 77.03 & 76.33 & 70.80 & 58.61\\
            \rowcolor{Gray!25}\textbf{DivideMix-Ours} & \textbf{77.42} & \textbf{77.21} & \textbf{72.41} & \textbf{64.02}\\
            % \hdashline
            % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.18}} & \scriptsize{\textbf{0.34}} & \scriptsize{\textbf{0.47}} & \scriptsize{\textbf{0.53}}\\
            \midrule
            InstanceGM~\cite{garg2023instance} & \textbf{79.69} & 79.21 & 78.47 & 77.19\\
            \rowcolor{Gray!25} \textbf{InstanceGM-Ours} & 79.61 & \textbf{79.40} & \textbf{79.52} & \textbf{77.76}\\
            % \hdashline
            % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.32}} & \scriptsize{\textbf{0.37}} & \scriptsize{\textbf{0.42}} & \scriptsize{\textbf{0.47}}\\
            \bottomrule
        \end{tabular}
    \end{subtable}
    \hfill
    % \begin{minipage}{.35\linewidth}
    %     \centering
    %     \begin{tabular}{l l l}
    %         \toprule
    %         \multirow{2}{*}{\small{\bfseries Actual Noise}} & \multicolumn{2}{c}{\small{\bfseries Estimated} \(\epsilon\)} \\
    %         \cmidrule{2 - 3} 
    %         & \tiny{\textbf{DivideMix}} & \tiny{\textbf{InstanceGM}} \\
    %         \midrule
    %         \textbf{0.2} & 0.18 & 0.32\\
    %         \textbf{0.3} & 0.34 & 0.37\\
    %         \textbf{0.4} & 0.47 & 0.42\\
    %         \textbf{0.5} & 0.53 & 0.47\\
    %         \bottomrule
    %     \end{tabular}
    % \end{minipage}
    % \begin{subtable}[t]{.4\linewidth}
    % \centering
    %  % \resizebox{\linewidth}{!}{
    %  \begin{tabular}{c c c}
    %     \toprule
    %     \multirow{2}{*}{\bfseries \shortstack{Actual\\Noise}} & \multicolumn{2}{c}{\bfseries Estimated noise rate} \\
    %     \cmidrule{2 - 3} 
    %     & \textbf{DivideMix} & \textbf{InstanceGM} \\
    %     \midrule
    %     0.2 & 0.18 & 0.32\\
    %     0.3 & 0.34 & 0.37\\
    %     0.4 & 0.47 & 0.42\\
    %     0.5 & 0.53 & 0.47\\
    %     \bottomrule
    % \end{tabular}
    % % }
% \end{subtable}
\begin{subtable}[t]{.45\linewidth}
        \centering
        \addtolength{\tabcolsep}{-0.1em}
        \begin{tabular}{l c c c c}
            \toprule
            \multicolumn{4}{l}{\bfseries Estimated noise rates} \\
            \midrule
            \multirow{2}{*}{\bfseries Method} & \multicolumn{4}{c}{\bfseries Actual noise rate} \\
            \cmidrule{2-5}
            & \bfseries 0.2 & \bfseries 0.3 & \bfseries 0.4 & \bfseries 0.5 \\
            \midrule
            DivideMix & 0.18 & 0.34 & 0.47 & 0.53 \\
            InstanceGM & 0.33 & 0.37 & 0.42 & 0.47 \\
            % \multirow{2}{*}{\bfseries \shortstack{Actual\\Noise}} & \multicolumn{3}{c}{\bfseries Estimated noise rate} \\
            % \cmidrule{2 - 4} 
            % & \textbf{DivideMix} & \textbf{InstanceGM} & \textbf{InstanceGM}-SS \\
            % \midrule
            % 0.4 & 0.39 & 0.38 & 0.48\\
            % 0.6 & 0.58 & 0.55 & 0.53\\
            % 0.8 & 0.73 & 0.74 & 0.69\\
            \bottomrule
        \end{tabular}
    \end{subtable}



\end{table}



==> csvs/clothing_table.tex <==
\begin{table}[t]
        \centering
        \caption{Test accuracy (\%) of competing methods, and final estimated noise rate $\epsilon$ on Clothing1M~\cite{xiao2015learning}.
        Also, we have not considered competing models that rely on a clean set whilst training.
        We integrate DivideMix~\cite{li2020dividemix}, SSR~\cite{feng2021ssr} and CC~\cite{zhao2022centrality} into our model. DivideMix~\cite{li2020dividemix} and CC~\cite{zhao2022centrality} shows the locally reproduced results. Estimated noise rate by~\cite{xiao2015learning} is \(0.385\). Our results are within \(1\%\) of the accuracy of the top approaches.}
        \label{table:clothing1M}
        \begin{tabular}{l c c}
            \toprule
            \bfseries Method & \bfseries Test accuracy (\%) & \bfseries Estimated noise rate \\
            \midrule
            % Nested-CoTeaching~\cite{chen2021boosting} & 74.90\\
            % CC~\cite{zhao2022centrality} & 75.40\\
            % MLC~\cite{zheng2021meta} & 75.78\\
            ELR+ with C2D~\cite{zheltonozhskii2022contrast} & 74.58\\
            AugDesc~\cite{nishi2021augmentation} & 75.11\\
            % DivideMix~\cite{li2020dividemix} & \textbf{74.76}\\
            \hline
            DivideMix~\cite{li2020dividemix} & 74.32\\
            \rowcolor{Gray!25}\textbf{DivideMix-Ours} & 74.41 & 0.41\\
            % AugDesc-WAW~\cite{nishi2021augmentation} & 74.72\\
            % AugDesc-WAW-Ours & 73.80 & 0.40\\
            \hline
            SSR (class-imbalance)~\cite{feng2021ssr} & 74.12 \\
            \rowcolor{Gray!25}\textbf{SSR-Ours}& 74.20 & 0.42\\
            \hline
            CC~\cite{feng2021ssr} & 75.24 \\
            \rowcolor{Gray!25}\textbf{CC-Ours}& \textbf{75.31} & 0.41\\
            \bottomrule
        \end{tabular}
\end{table}

==> csvs/f1_OursDM.tex <==
epochs	F1
251	0.7892001848
252	0.8038617135
253	0.800317608
254	0.814220749
255	0.8092667537
256	0.8196632402
257	0.817145849
258	0.8251670558
259	0.8280925179
260	0.8306206187
261	0.8347457619
262	0.8397424437
263	0.8397057414
264	0.847228216
265	0.8454640934
266	0.8506409096
267	0.8511484807
268	0.860264306
269	0.8577240772
270	0.8678396243
271	0.8619175478
272	0.8734077393
273	0.8677531803
274	0.8770688967
275	0.8748660606
276	0.8839559308
277	0.8828349712
278	0.8885166025
279	0.8847485719
280	0.8886467761
281	0.8875531094
282	0.8947460545
283	0.8915533139
284	0.8936685436
285	0.893821577
286	0.9015310616
287	0.8941770533
288	0.9008817506
289	0.8967950185
290	0.9030303547
291	0.8923716047
292	0.8988280148
293	0.8989553115
294	0.8928943441
295	0.8954656275
296	0.8982876277
297	0.8960902273
298	0.8937003007
299	0.8941168553
300	0.895376751
% epochs	F1
% 30	0.4561081707
% 31	0.5662687015
% 32	0.6116046744
% 33	0.6524676786
% 34	0.6691067313
% 35	0.679749608
% 36	0.6974871166
% 37	0.6965648921
% 38	0.7100132391
% 39	0.7102583879
% 40	0.7190988888
% 41	0.7202563065
% 42	0.7291313239
% 43	0.7302640467
% 44	0.7401839101
% 45	0.7393757841
% 46	0.7499485282
% 47	0.7433547502
% 48	0.7607161854
% 49	0.7512526808
% 50	0.7711383536
% 51	0.7619538396
% 52	0.7779005213
% 53	0.7754081094
% 54	0.7887853458
% 55	0.7847293648
% 56	0.7946951851
% 57	0.7892001848
% 58	0.8038617135
% 59	0.800317608
% 60	0.814220749
% 61	0.8092667537
% 62	0.8196632402
% 63	0.817145849
% 64	0.8251670558
% 65	0.8280925179
% 66	0.8306206187
% 67	0.8347457619
% 68	0.8397424437
% 69	0.8397057414
% 70	0.847228216
% 71	0.8454640934
% 72	0.8506409096
% 73	0.8511484807
% 74	0.860264306
% 75	0.8577240772
% 76	0.8678396243
% 77	0.8619175478
% 78	0.8734077393
% 79	0.8677531803
% 80	0.8770688967
% 81	0.8748660606
% 82	0.8839559308
% 83	0.8828349712
% 84	0.8885166025
% 85	0.8847485719
% 86	0.8886467761
% 87	0.8875531094
% 88	0.8947460545
% 89	0.8915533139
% 90	0.8936685436
% 91	0.893821577
% 92	0.9015310616
% 93	0.8941770533
% 94	0.9008817506
% 95	0.8967950185
% 96	0.9030303547
% 97	0.8923716047
% 98	0.8988280148
% 99	0.8989553115
% 100	0.8928943441

==> csvs/f1_OursSSR.tex <==
epochs F1
251	0.9190500379
252	0.9185315967
253	0.9157599211
254	0.9197832942
255	0.918915689
256	0.9179045558
257	0.9190420508
258	0.9186763167
259	0.9198340178
260	0.9185382724
261	0.9162952304
262	0.922056675
263	0.9206113815
264	0.9250764346
265	0.9226144552
266	0.9255012369
267	0.9210367799
268	0.923040092
269	0.9214970469
270	0.9294380045
271	0.9205724597
272	0.9286185598
273	0.9221510887
274	0.9241014123
275	0.9248276949
276	0.9241041541
277	0.9232239723
278	0.9254823923
279	0.9252516031
280	0.924489677
281	0.9225981832
282	0.9253737926
283	0.925365448
284	0.9243163466
285	0.9288290834
286	0.9252096415
287	0.9270761609
288	0.9277262092
289	0.9269922376
290	0.9251800275
291	0.9271333218
292	0.9213260412
293	0.9286246896
294	0.9274109602
295	0.9218652844
296	0.9196243382
297	0.9240685701
298	0.9238212705
299	0.9278346896
300	0.9246950245


==> csvs/f1_dm.tex <==
epochs	F1
251	0.7683591999
252	0.7664094569
253	0.767946362
254	0.7662260954
255	0.7669812502
256	0.766278262
257	0.7678487862
258	0.7658302418
259	0.768090966
260	0.7680999229
261	0.7671453415
262	0.7676463907
263	0.7673628201
264	0.767588086
265	0.7677670082
266	0.7683674104
267	0.767595499
268	0.7677588177
269	0.7667914899
270	0.7664797388
271	0.7672837342
272	0.7669671023
273	0.7683399074
274	0.7677807523
275	0.7667769565
276	0.7675885002
277	0.7683694644
278	0.7664126831
279	0.7678507686
280	0.7680440764
281	0.7678195116
282	0.7681812923
283	0.7680391105
284	0.7680734797
285	0.769523832
286	0.7673157353
287	0.7679783014
288	0.7678569341
289	0.7675302173
290	0.7671082824
291	0.767751244
292	0.7680185928
293	0.7680379445
294	0.768338849
295	0.7674358106
296	0.7684660378
297	0.7696180755
298	0.7691715368
299	0.7693023369
300	0.7679781579













% epochs	F1
% 30	0.6828992291
% 31	0.716003771
% 32	0.7387447093
% 33	0.7487636502
% 34	0.7472515175
% 35	0.7534645191
% 36	0.7510976775
% 37	0.7570090148
% 38	0.7571910873
% 39	0.7584667242
% 40	0.7582814516
% 41	0.7615102111
% 42	0.7585898283
% 43	0.7598755795
% 44	0.7553902295
% 45	0.7575273978
% 46	0.7593399813
% 47	0.7589992131
% 48	0.754230891
% 49	0.7603295266
% 50	0.7478692832
% 51	0.7554704659
% 52	0.7568136724
% 53	0.7599417344
% 54	0.7587393379
% 55	0.7601856876
% 56	0.7596111657
% 57	0.7587914744
% 58	0.7581041957
% 59	0.7586308424
% 60	0.7572335485
% 61	0.7579597614
% 62	0.7609452815
% 63	0.7581360103
% 64	0.7570970494
% 65	0.7602690706
% 66	0.7597444243
% 67	0.7598171525
% 68	0.7573108273
% 69	0.7608769655
% 70	0.7608566965
% 71	0.7586739851
% 72	0.7582496687
% 73	0.757998878
% 74	0.7623966499
% 75	0.7590953658
% 76	0.7597278763
% 77	0.7591086176
% 78	0.7591047865
% 79	0.7565881698
% 80	0.7600337404
% 81	0.7616021493
% 82	0.7573055414
% 83	0.7584518812
% 84	0.7569094235
% 85	0.7580005757
% 86	0.7600532713
% 87	0.7624712659
% 88	0.7603194407
% 89	0.7625229983
% 90	0.7397066189
% 91	0.7612403351
% 92	0.7606900897
% 93	0.7583490413
% 94	0.7577882681
% 95	0.7610103464
% 96	0.7591702667
% 97	0.7624950775
% 98	0.7604567651
% 99	0.7625810783
% 100	0.7629366648
% 101	0.7593711554
% 102	0.7611597305
% 103	0.763118554
% 104	0.7616071109
% 105	0.7623772608
% 106	0.7619187888
% 107	0.7614280308
% 108	0.7605253588
% 109	0.7618332856
% 110	0.7625505859
% 111	0.7604042376
% 112	0.7633390243
% 113	0.7645371691
% 114	0.7627777024
% 115	0.7630486411
% 116	0.7621534216
% 117	0.7609193027
% 118	0.764717161
% 119	0.7637002547
% 120	0.7629915099
% 121	0.7615470891
% 122	0.7653147703
% 123	0.7633203593
% 124	0.7616344103
% 125	0.7613025935
% 126	0.7649353411
% 127	0.7635859056
% 128	0.7645827979
% 129	0.7673932668
% 130	0.764836002
% 131	0.7647337136
% 132	0.7630702654
% 133	0.7631756298
% 134	0.7668966127
% 135	0.7632556234
% 136	0.7654434124
% 137	0.7636210693
% 138	0.7644085967
% 139	0.7627970546
% 140	0.7656171111
% 141	0.7646713973
% 142	0.7661489995
% 143	0.767152258
% 144	0.7632243246
% 145	0.7695204863
% 146	0.7649071063
% 147	0.7642780922
% 148	0.7644169422
% 149	0.7634082583
% 150	0.7647796566
% 151	0.7663011034
% 152	0.7666932248
% 153	0.7671039156
% 154	0.766325376
% 155	0.7670104966
% 156	0.7671886491
% 157	0.7672438343
% 158	0.766456076
% 159	0.767454966
% 160	0.7667614425
% 161	0.7678404329
% 162	0.7665733764
% 163	0.7668659106
% 164	0.7672187264
% 165	0.7674475469
% 166	0.7669930375
% 167	0.7677198197
% 168	0.767250847
% 169	0.7673679507
% 170	0.766284385
% 171	0.7662901853
% 172	0.7668869841
% 173	0.767266497
% 174	0.7666163295
% 175	0.7666254629
% 176	0.7666072702
% 177	0.7667191738
% 178	0.7675686827
% 179	0.7664023294
% 180	0.76732236
% 181	0.7670448939
% 182	0.7666391418
% 183	0.7685746531
% 184	0.766724654
% 185	0.767732401
% 186	0.7685257554
% 187	0.767187436
% 188	0.7665632597
% 189	0.7651779835
% 190	0.7675908176
% 191	0.7676762318
% 192	0.7678096331
% 193	0.7676226259
% 194	0.7667696238
% 195	0.7667951625
% 196	0.7668603497
% 197	0.7671126548
% 198	0.7686108193
% 199	0.7681040986
% 200	0.7673145143
% 201	0.7679932273
% 202	0.7663086583
% 203	0.766411961
% 204	0.766475
% 205	0.767809148
% 206	0.7673793628
% 207	0.7675259314
% 208	0.7668991931
% 209	0.7674622277
% 210	0.7669392449
% 211	0.7673596953
% 212	0.7675978137
% 213	0.7668186997
% 214	0.7658190568
% 215	0.7669738041
% 216	0.7658336497
% 217	0.767046763
% 218	0.7675749122
% 219	0.7668147041
% 220	0.7672596741
% 221	0.7673678597
% 222	0.7668883306
% 223	0.7674197367
% 224	0.7663623951
% 225	0.7672221229
% 226	0.7669503886
% 227	0.7671006758
% 228	0.7668796222
% 229	0.7673383259
% 230	0.7679908172
% 231	0.7670049305
% 232	0.7671063182
% 233	0.7676685725
% 234	0.7682769381
% 235	0.7661865066
% 236	0.7681579742
% 237	0.7685757972
% 238	0.7670240059
% 239	0.7672799242
% 240	0.7677765469
% 241	0.7674699485
% 242	0.7665015331
% 243	0.766230491
% 244	0.7673762367
% 245	0.7669397966
% 246	0.7673772301
% 247	0.7671403035
% 248	0.7673139807
% 249	0.7685484087
% 250	0.7671931073
% 251	0.7683591999
% 252	0.7664094569
% 253	0.767946362
% 254	0.7662260954
% 255	0.7669812502
% 256	0.766278262
% 257	0.7678487862
% 258	0.7658302418
% 259	0.768090966
% 260	0.7680999229
% 261	0.7671453415
% 262	0.7676463907
% 263	0.7673628201
% 264	0.767588086
% 265	0.7677670082
% 266	0.7683674104
% 267	0.767595499
% 268	0.7677588177
% 269	0.7667914899
% 270	0.7664797388
% 271	0.7672837342
% 272	0.7669671023
% 273	0.7683399074
% 274	0.7677807523
% 275	0.7667769565
% 276	0.7675885002
% 277	0.7683694644
% 278	0.7664126831
% 279	0.7678507686
% 280	0.7680440764
% 281	0.7678195116
% 282	0.7681812923
% 283	0.7680391105
% 284	0.7680734797
% 285	0.769523832
% 286	0.7673157353
% 287	0.7679783014
% 288	0.7678569341
% 289	0.7675302173
% 290	0.7671082824
% 291	0.767751244
% 292	0.7680185928
% 293	0.7680379445
% 294	0.768338849
% 295	0.7674358106
% 296	0.7684660378
% 297	0.7696180755
% 298	0.7691715368
% 299	0.7693023369
% 300	0.7679781579

==> csvs/f1_ssr.tex <==
epochs F1
251	0.9334147573
252	0.9351729155
253	0.9338775277
254	0.9351419806
255	0.9347442985
256	0.9360863566
257	0.9365566373
258	0.9346481562
259	0.9355261922
260	0.9370458722
261	0.9360802174
262	0.9369777441
263	0.9351744056
264	0.9378361106
265	0.9356426001
266	0.9349445701
267	0.9372436404
268	0.936748147
269	0.9374577999
270	0.9355550408
271	0.9341064095
272	0.934443295
273	0.9346714616
274	0.9353333116
275	0.9362196922
276	0.9352291226
277	0.9350890517
278	0.9368373156
279	0.9358764291
280	0.9377340078
281	0.936524868
282	0.9366203547
283	0.9373795986
284	0.9365481138
285	0.9366309047
286	0.9389259815
287	0.9379139543
288	0.937071979
289	0.9379037023
290	0.9370123744
291	0.9361744523
292	0.9372850657
293	0.9369889498
294	0.9377762675
295	0.9368312955
296	0.9381513
297	0.9372287393
298	0.9388841391
299	0.9378929138

==> csvs/miniwebvision_table.tex <==
% \begin{table}[t]
%         \caption{Test accuracy (\%) on mini-WebVision~\cite{li2020dividemix} and validation on ImageNet~\cite{krizhevsky2012imagenet}. Base model is Contrast-to-Divide(C2D)~\cite{zheltonozhskii2022contrast} represented by \(*\) with results in \textit{italics}, whilst \textbf{C2D-Ours} is our proposed results. ImageNet~\cite{krizhevsky2012imagenet} is only considered for validation so noise rate is not estimated on that.
%         }
%         \label{table:miniWebvision}
%         \centering
%         \begin{tabular}{l c c c c c}
%         \toprule
%         \multirow{2}{*}{\bfseries Dataset} & \multicolumn{2}{c}{\bfseries mini-WebVision} & \multicolumn{2}{c}{\bfseries ImageNet} & {\bfseries Estimated \(\epsilon\)} &
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
%         & \textbf{Top-1} & \textbf{Top-5} & \textbf{Top-1} & \textbf{Top-5} \\
%         \midrule
%         DivideMix~\cite{li2020dividemix}  & 77.32 & 91.64 & 75.20 & 91.64 & \\
%         BtR~\cite{smart2023bootstrapping} & 80.88 & 92.76 & 75.96 & 92.20 & \\
%         SSR~\cite{feng2021ssr} & \textbf{80.92} & \textbf{92.80} & 75.76 & 91.76 & \\
%         \midrule
%         C2D*~\cite{zheltonozhskii2022contrast} & \textit{79.42} & \textit{92.32} & \textit{78.57} & \textit{93.04} & \\
%         \rowcolor{Gray!25}\textbf{C2D-Ours}  & 79.31 & 92.28 & \textbf{79.16} & \textbf{93.12} & \textbf{0.43} \\
%         % \hdashline
%         % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.43}} & & & \\
%         \bottomrule
%         \end{tabular}
% \end{table} 
\begin{table}[t]
    \caption{Test accuracy (\%) and final estimated noise rate \(\epsilon\) on mini-WebVision~\cite{li2020dividemix} and validation on ImageNet~\cite{krizhevsky2012imagenet}. We integrate Contrast-to-Divide (C2D)~\cite{zheltonozhskii2022contrast} into our model, whilst \textbf{C2D-Ours} is our proposed approach. ImageNet~\cite{krizhevsky2012imagenet} is only considered for validation.}
    \label{table:miniWebvision}
    \centering
    \begin{tabular}{l c c c c c}
        \toprule
        \multirow{2}{*}{\bfseries Dataset} & \multicolumn{2}{c}{\bfseries mini-WebVision} & \multicolumn{2}{c}{\bfseries ImageNet} & \multirow{2}{*}{\bfseries Estimated noise rate} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & \textbf{Top-1} & \textbf{Top-5} & \textbf{Top-1} & \textbf{Top-5} & \\
        \midrule
        DivideMix~\cite{li2020dividemix}  & 77.32 & 91.64 & 75.20 & 91.64 & \\
        BtR~\cite{smart2023bootstrapping} & 80.88 & 92.76 & 75.96 & 92.20 & \\
        SSR~\cite{feng2021ssr} & \textbf{80.92} & 92.80 & 75.76 & 91.76 & \\
        \midrule
        C2D~\cite{zheltonozhskii2022contrast} & 79.42 & 92.32 & 78.57 & 93.04 & \\
        \rowcolor{Gray!25}\textbf{C2D-Ours}  & 80.20 & \textbf{92.82} & \textbf{79.16} & \textbf{93.12} & \textbf{0.43} \\
        % \hdashline
        % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.43}} & & & \\
        \bottomrule
    \end{tabular}
\end{table}


==> csvs/motivation.tex <==
epochs,DivideMix,fixE
50,56.68,59.88
51,56.43,59.88
52,58.25,60.29
53,57.41,60.29
54,56.34,60.29
55,58.01,60.29
56,57.92,60.29
57,58.78,60.29
58,59.61,60.29
59,57.66,60.29
60,57.75,60.29
61,54.82,60.29
62,56.13,60.29
63,57.21,60.68
64,56.82,60.68
65,57.61,60.68
66,56.69,60.68
67,57.67,60.68
68,57.86,61.03
69,56.31,61.03
70,56.49,61.03
71,57.57,61.03
72,56.75,61.03
73,56.48,61.03
74,57.26,61.03
75,57.09,61.03
76,58.07,61.03
77,58.24,61.03
78,58.52,61.03
79,57.14,61.03
80,59.06,61.03
81,56.96,61.03
82,56.52,61.03
83,56.74,61.03
84,58.08,61.03
85,57.22,61.03
86,57.79,61.03
87,58.81,62.38
88,57.48,62.38
89,58.54,62.38
90,57.03,62.38
91,58.68,62.38
92,57.94,62.38
93,56.75,62.38
94,56.93,62.38
95,57.43,62.38
96,58.15,62.38
97,56.95,62.38
98,58.62,62.38
99,59.39,62.38
100,58.22,62.38
101,60.2,62.38
102,58.81,62.38
103,59.76,62.38
104,58.07,62.77
105,57.79,62.77
106,57.77,62.77
107,57.48,62.77
108,58.56,62.77
109,56,62.77
110,58.55,62.77
111,55.96,62.77
112,58.91,62.77
113,57.97,62.77
114,57.52,62.77
115,57.65,62.77
116,59.58,63.54
117,58.73,63.54
118,59.34,63.54
119,58.43,63.54
120,59.52,63.54
121,55.86,63.54
122,57.5,63.54
123,57.02,63.54
124,57.99,63.54
125,59.11,63.54
126,59.55,63.54
127,57.36,63.54
128,57.84,63.54
129,57.09,63.54
130,58.75,63.54
131,58.08,63.54
132,59.28,63.54
133,56.97,63.54
134,58.24,63.54
135,57.84,63.54
136,57.73,63.54
137,59.17,63.54
138,59.1,63.54
139,58.29,63.54
140,59.13,63.54
141,58.13,63.54
142,57.59,63.54
143,56.57,63.54
144,58.46,63.54
145,60.45,63.54
146,59.25,63.54
147,57.56,63.54
148,58.04,63.54
149,59.79,63.54
150,59.04,63.54
151,59.13,63.54
152,58.59,63.54
153,58.82,63.54
154,58.34,63.54
155,57.7,63.54
156,58.42,63.54
157,57.92,63.54
158,57.44,63.54
159,57.74,63.54
160,57.48,63.54
161,58.23,63.54
162,57.76,63.54
163,57.68,63.54
164,57.54,63.54
165,56.72,63.54
166,56.56,63.54
167,56.86,63.54
168,57.16,63.54
169,57.07,63.54
170,57.45,63.54
171,56.97,63.54
172,57.6,63.54
173,57.06,63.54
174,56.84,63.54
175,57.76,63.54
176,57.22,63.54
177,57.66,63.54
178,57.19,63.54
179,56.44,63.54
180,57.1,63.54
181,57.4,63.54
182,57.33,63.54
183,57.58,63.54
184,57.26,63.54
185,56.75,63.54
186,57.36,63.54
187,57.32,63.54
188,56.83,63.54
189,56.63,63.54
190,57.65,63.54
191,58.58,63.54
192,57.7,63.54
193,57.09,63.54
194,57.3,63.54
195,57.81,63.54
196,57.52,63.54
197,57.59,63.54
198,58.65,63.54
199,57.52,63.54
200,57.35,63.54
201,57.3,63.54
202,57.17,63.54
203,58.45,63.54
204,57.72,63.54
205,58.03,63.54
206,57.38,63.54
207,57.93,63.54
208,56.36,63.54
209,58.01,63.54
210,57.62,63.54
211,57.63,63.54
212,57.61,63.54
213,57.32,63.54
214,56.61,63.54
215,58.44,63.54
216,58.79,63.54
217,58.22,63.54
218,56.96,63.54
219,57.46,63.61
220,58.18,63.61
221,57.22,63.78
222,57.17,63.78
223,57.6,63.78
224,57.64,63.78
225,56.98,63.78
226,58.36,63.78
227,58.6,63.78
228,57.66,63.78
229,57.08,63.78
230,57.74,63.78
231,57.3,63.82
232,57.03,63.9
233,58.22,64.1
234,58.26,64.1
235,58.52,64.1
236,57.67,64.1
237,58.25,64.1
238,57.32,64.1
239,57.07,64.1
240,56.59,64.1
241,56.56,64.1
242,57.9,64.1
243,57.58,64.1
244,57.86,64.1
245,58.3,64.1
246,58.25,64.1
247,57.37,64.12
248,57.85,64.12
249,58.24,64.12
250,57.8,64.12
251,57.39,64.12
252,58.43,64.12
253,58.25,64.12
254,58.39,64.12
255,58.2,64.12
256,57.61,64.12
257,57.55,64.12
258,58.61,64.12
259,56.35,64.12
260,56.37,64.12
261,57.46,64.12
262,57.34,64.12
263,57.2,64.12
264,57.3,64.12
265,57.74,64.12
266,57.14,64.41
267,57.84,64.44
268,57.85,64.44
269,57.9,64.44
270,58.66,64.44
271,57.49,64.44
272,58.42,64.44
273,58.02,64.44
274,58.84,64.44
275,57.38,64.44
276,57.68,64.44
277,57.97,64.44
278,57.06,64.44
279,58.28,64.44
280,57.64,64.44
281,58.18,64.44
282,57.97,64.44
283,57.48,64.44
284,58.11,64.44
285,58.13,64.44
286,57.29,64.44
287,57.86,64.44
288,58.77,64.44
289,57.86,64.44
290,56.6,64.44
291,56.75,64.44
292,57.75,64.44
293,57.3,64.44
294,57.53,64.44
295,57.39,64.44
296,57.62,64.44
297,58.06,64.44
298,57.91,64.44
299,58.58,64.44
300,57.3,64.44

==> csvs/precision_OursDM.tex <==
epochs	Precision
251	0.9191807267
252	0.9172946209
253	0.9321553806
254	0.9285749161
255	0.9369454112
256	0.9293250398
257	0.9379312351
258	0.93151795
259	0.9394985416
260	0.9329482419
261	0.9425024227
262	0.9331171543
263	0.9470869682
264	0.9303998795
265	0.9500115276
266	0.93277893
267	0.9462518582
268	0.9389959593
269	0.9529942419
270	0.9396757385
271	0.9494444119
272	0.9414629844
273	0.9504003964
274	0.940260932
275	0.954094698
276	0.940904147
277	0.9520851162
278	0.9399962934
279	0.9475617557
280	0.9456566723
281	0.9456121125
282	0.9449918466
283	0.9473507027
284	0.940747904
285	0.9477447577
286	0.9398687969
287	0.9428883457
288	0.9380672507
289	0.9400097177
290	0.9332818249
291	0.9421172043
292	0.9325772435
293	0.9378661503
294	0.929061979
295	0.9357523338
296	0.9252759878
297	0.9362514262
298	0.9298602439
299	0.9326635401
300	0.9326630001

% epochs	Precision
% 30	0.639442372
% 31	0.7595786969
% 32	0.8533910673
% 33	0.8695127245
% 34	0.9018902446
% 35	0.9191807267
% 36	0.9172946209
% 37	0.9321553806
% 38	0.9285749161
% 39	0.9369454112
% 40	0.9293250398
% 41	0.9379312351
% 42	0.93151795
% 43	0.9394985416
% 44	0.9329482419
% 45	0.9425024227
% 46	0.9331171543
% 47	0.9470869682
% 48	0.9303998795
% 49	0.9500115276
% 50	0.93277893
% 51	0.9462518582
% 52	0.9389959593
% 53	0.9529942419
% 54	0.9396757385
% 55	0.9494444119
% 56	0.9414629844
% 57	0.9504003964
% 58	0.940260932
% 59	0.954094698
% 60	0.940904147
% 61	0.9520851162
% 62	0.9399962934
% 63	0.9475617557
% 64	0.9456566723
% 65	0.9456121125
% 66	0.9449918466
% 67	0.9473507027
% 68	0.940747904
% 69	0.9477447577
% 70	0.9398687969
% 71	0.9428883457
% 72	0.9380672507
% 73	0.9400097177
% 74	0.9332818249
% 75	0.9421172043
% 76	0.9325772435
% 77	0.9378661503
% 78	0.929061979
% 79	0.9357523338
% 80	0.9252759878
% 81	0.9362514262
% 82	0.9298602439
% 83	0.9326635401
% 84	0.9233139078
% 85	0.9284185928
% 86	0.920992562
% 87	0.9250521573
% 88	0.9184765846
% 89	0.9183151601
% 90	0.9112639058
% 91	0.9187074945
% 92	0.9086629449
% 93	0.9139611602
% 94	0.9039073673
% 95	0.9067873581
% 96	0.896612206
% 97	0.8994552527
% 98	0.8911890566
% 99	0.8896207431
% 100	0.8875452081

==> csvs/precision_OursSSR.tex <==
epochs Precision 
251	0.9604756236
252	0.9593145847
253	0.9667548537
254	0.9625743628
255	0.9680587649
256	0.9655769467
257	0.9698451257
258	0.9623534083
259	0.9672937489
260	0.9647271633
261	0.9596340656
262	0.9646325707
263	0.9645869136
264	0.9646216631
265	0.9652692676
266	0.965223074
267	0.9655439854
268	0.9630112648
269	0.9652463794
270	0.9636149406
271	0.9632848501
272	0.9655144215
273	0.9618096447
274	0.9697117305
275	0.9633510113
276	0.9638339877
277	0.9609236121
278	0.961569488
279	0.9641461372
280	0.9645846486
281	0.9627708793
282	0.9640131593
283	0.9633671641
284	0.962844193
285	0.9638023376
286	0.9610800147
287	0.9610789418
288	0.9611592293
289	0.9623958468
290	0.9609194398
291	0.9629098773
292	0.9603625536
293	0.9615155458
294	0.9611188173
295	0.9611588717
296	0.9606446028
297	0.9589826465
298	0.9608424306
299	0.9604483843
300	0.9611213803

==> csvs/precision_dm.tex <==
epochs	Precision
251	0.6758604109
252	0.6742550735
253	0.6758700558
254	0.6747137021
255	0.6749782213
256	0.6744228382
257	0.6756957201
258	0.6739144346
259	0.6753068201
260	0.6760847644
261	0.67495414
262	0.6755445822
263	0.6751981709
264	0.6749450669
265	0.6761031884
266	0.6761511113
267	0.6755353402
268	0.6750242513
269	0.6746611718
270	0.6748744694
271	0.6755630835
272	0.6741006379
273	0.675923152
274	0.6755208326
275	0.6747545685
276	0.6754317377
277	0.6762238747
278	0.6750729707
279	0.6757683731
280	0.6757431553
281	0.6753955661
282	0.6762805462
283	0.6754114727
284	0.6760437913
285	0.6772464833
286	0.6753339675
287	0.6750403661
288	0.6756851518
289	0.6756198731
290	0.6746653013
291	0.6755214901
292	0.675889149
293	0.6758263638
294	0.6757363843
295	0.6754039696
296	0.6762111092
297	0.6775782927
298	0.6767240979
299	0.6771586117
300	0.6753403165
% epochs	Precision
% 30	0.5635498939
% 31	0.6364757212
% 32	0.6483247384
% 33	0.6615357824
% 34	0.6648715854
% 35	0.6688135312
% 36	0.6634082004
% 37	0.6699483046
% 38	0.665222808
% 39	0.6697871596
% 40	0.6661005532
% 41	0.6705171081
% 42	0.6653153914
% 43	0.6701488944
% 44	0.6629966378
% 45	0.6671317326
% 46	0.6668373221
% 47	0.6645569014
% 48	0.6615090709
% 49	0.6663032955
% 50	0.6599058001
% 51	0.6626626519
% 52	0.6639071992
% 53	0.6648928752
% 54	0.663706758
% 55	0.6647475899
% 56	0.6649289513
% 57	0.6646237
% 58	0.6640229893
% 59	0.6639018764
% 60	0.662869147
% 61	0.6635974514
% 62	0.6651888559
% 63	0.6637770668
% 64	0.6658618805
% 65	0.6637085186
% 66	0.665405142
% 67	0.6640942867
% 68	0.6646269423
% 69	0.6645684427
% 70	0.6717236622
% 71	0.6643754226
% 72	0.6677401059
% 73	0.6660786298
% 74	0.6666426997
% 75	0.6644100293
% 76	0.6678736974
% 77	0.6671474746
% 78	0.6671876648
% 79	0.6655372571
% 80	0.6707940299
% 81	0.6682375379
% 82	0.6679313547
% 83	0.6660417336
% 84	0.6641460722
% 85	0.6682163314
% 86	0.6666307074
% 87	0.6721489512
% 88	0.6674524714
% 89	0.6680575026
% 90	0.6624292255
% 91	0.6690343989
% 92	0.6665841569
% 93	0.6682671869
% 94	0.6670015748
% 95	0.6716808137
% 96	0.6684699747
% 97	0.672045741
% 98	0.6710065246
% 99	0.6694249133
% 100	0.672896054
% 101	0.6714596291
% 102	0.671937122
% 103	0.6737430334
% 104	0.6715306672
% 105	0.6728935808
% 106	0.6725789848
% 107	0.6729692636
% 108	0.6713248919
% 109	0.6733894683
% 110	0.6713165164
% 111	0.6709247349
% 112	0.6729833305
% 113	0.6731412245
% 114	0.6718781143
% 115	0.6734223824
% 116	0.6725449053
% 117	0.6701124502
% 118	0.6742135078
% 119	0.675360329
% 120	0.6742762408
% 121	0.6696008018
% 122	0.6741612396
% 123	0.6691002385
% 124	0.6730078458
% 125	0.6703346924
% 126	0.6758463376
% 127	0.6738597899
% 128	0.6734912486
% 129	0.6771586005
% 130	0.6757857399
% 131	0.6741924609
% 132	0.6708933364
% 133	0.6735967121
% 134	0.6769725194
% 135	0.6719446875
% 136	0.6751557244
% 137	0.6728142484
% 138	0.6738975608
% 139	0.6739253266
% 140	0.6760608242
% 141	0.6738619887
% 142	0.6784101728
% 143	0.6775124285
% 144	0.6734610861
% 145	0.681215427
% 146	0.675920407
% 147	0.6745855437
% 148	0.6747078324
% 149	0.6734892622
% 150	0.6718052742
% 151	0.6743190427
% 152	0.6741158326
% 153	0.6743351164
% 154	0.6741017814
% 155	0.6738221523
% 156	0.674189323
% 157	0.674044271
% 158	0.6737492474
% 159	0.6748547464
% 160	0.6744757058
% 161	0.6746200387
% 162	0.6733775334
% 163	0.6742673385
% 164	0.6738905197
% 165	0.675051404
% 166	0.6734734735
% 167	0.6743648492
% 168	0.6746315265
% 169	0.6739598587
% 170	0.6741541119
% 171	0.6737005703
% 172	0.6736085359
% 173	0.674424863
% 174	0.6749235249
% 175	0.6746126971
% 176	0.6745613385
% 177	0.6746419013
% 178	0.675007507
% 179	0.6739663855
% 180	0.6744650508
% 181	0.6743362128
% 182	0.6741477277
% 183	0.676031811
% 184	0.6748591529
% 185	0.6760727791
% 186	0.6757942951
% 187	0.6747877623
% 188	0.673984183
% 189	0.6739256994
% 190	0.6752036787
% 191	0.675243279
% 192	0.6750335347
% 193	0.6749753724
% 194	0.6744652211
% 195	0.6748059583
% 196	0.675208865
% 197	0.674996228
% 198	0.6768535409
% 199	0.675627659
% 200	0.6754481492
% 201	0.6757339423
% 202	0.6739370978
% 203	0.6746996759
% 204	0.6741713134
% 205	0.675634333
% 206	0.6756648563
% 207	0.6757758658
% 208	0.6755717048
% 209	0.6754448929
% 210	0.6746582782
% 211	0.6752396938
% 212	0.6753071233
% 213	0.6744023399
% 214	0.6743383237
% 215	0.6746886132
% 216	0.6740589074
% 217	0.6744083736
% 218	0.6757123668
% 219	0.6747434707
% 220	0.6748069931
% 221	0.6752291542
% 222	0.6746489366
% 223	0.6759136062
% 224	0.6745764089
% 225	0.6757932882
% 226	0.6750928574
% 227	0.675349015
% 228	0.6744734595
% 229	0.6752297852
% 230	0.6765668711
% 231	0.6757358282
% 232	0.67556706
% 233	0.6757413962
% 234	0.6763823368
% 235	0.6746523103
% 236	0.6755953384
% 237	0.6762188235
% 238	0.6749980576
% 239	0.6754177665
% 240	0.6756766003
% 241	0.6757355619
% 242	0.6750711167
% 243	0.6743720352
% 244	0.6757065146
% 245	0.6748444564
% 246	0.6751046356
% 247	0.6754104474
% 248	0.675749545
% 249	0.6762923025
% 250	0.6750049217
% 251	0.6758604109
% 252	0.6742550735
% 253	0.6758700558
% 254	0.6747137021
% 255	0.6749782213
% 256	0.6744228382
% 257	0.6756957201
% 258	0.6739144346
% 259	0.6753068201
% 260	0.6760847644
% 261	0.67495414
% 262	0.6755445822
% 263	0.6751981709
% 264	0.6749450669
% 265	0.6761031884
% 266	0.6761511113
% 267	0.6755353402
% 268	0.6750242513
% 269	0.6746611718
% 270	0.6748744694
% 271	0.6755630835
% 272	0.6741006379
% 273	0.675923152
% 274	0.6755208326
% 275	0.6747545685
% 276	0.6754317377
% 277	0.6762238747
% 278	0.6750729707
% 279	0.6757683731
% 280	0.6757431553
% 281	0.6753955661
% 282	0.6762805462
% 283	0.6754114727
% 284	0.6760437913
% 285	0.6772464833
% 286	0.6753339675
% 287	0.6750403661
% 288	0.6756851518
% 289	0.6756198731
% 290	0.6746653013
% 291	0.6755214901
% 292	0.675889149
% 293	0.6758263638
% 294	0.6757363843
% 295	0.6754039696
% 296	0.6762111092
% 297	0.6775782927
% 298	0.6767240979
% 299	0.6771586117
% 300	0.6753403165

==> csvs/precision_ssr.tex <==
epochs Precision
251	0.9567984939
252	0.9569339752
253	0.9568281174
254	0.9577544332
255	0.9575598836
256	0.9571226835
257	0.9575554132
258	0.9573323727
259	0.9571070075
260	0.9575993419
261	0.9576717615
262	0.95732373
263	0.9578372836
264	0.9572612047
265	0.9557207227
266	0.9551900029
267	0.9569969177
268	0.956271112
269	0.9551798105
270	0.9576991796
271	0.9573637843
272	0.9558490515
273	0.954618752
274	0.9543943405
275	0.9553722143
276	0.9546069503
277	0.9557690024
278	0.9544302225
279	0.9558720589
280	0.9537459016
281	0.9534670711
282	0.9524350166
283	0.9533153772
284	0.954326272
285	0.9536729455
286	0.95359236
287	0.9536985159
288	0.9543688893
289	0.9543136954
290	0.9546797872
291	0.9534804821
292	0.9535549879
293	0.953686595
294	0.9526460767
295	0.9535401464
296	0.9535197616
297	0.9534051418
298	0.9527698159
299	0.9535859227

==> csvs/ratio_OursDM.tex <==
epochs	Ratio
251	0.36206
252	0.3655
253	0.3687
254	0.3719
255	0.37518
256	0.37858
257	0.38194
258	0.3853
259	0.3889
260	0.39242
261	0.39588
262	0.39942
263	0.403
264	0.4067
265	0.41036
266	0.414
267	0.4177
268	0.42142
269	0.4251
270	0.42898
271	0.43274
272	0.43664
273	0.4406
274	0.44448
275	0.44834
276	0.45226
277	0.45616
278	0.46014
279	0.46416
280	0.46818
281	0.47214
282	0.47618
283	0.48028
284	0.48424
285	0.48816
286	0.49214
287	0.4963
288	0.50026
289	0.50426
290	0.50832
291	0.51246
292	0.5165
293	0.5206
294	0.52464
295	0.52868
296	0.53272
297	0.5367
298	0.54088
299	0.54484
300	0.54888
% epochs	Ratio
% 30	0.28292
% 31	0.28694
% 32	0.28942
% 33	0.292
% 34	0.2945
% 35	0.29708
% 36	0.29982
% 37	0.3025
% 38	0.30534
% 39	0.30806
% 40	0.31082
% 41	0.31364
% 42	0.31642
% 43	0.31922
% 44	0.32214
% 45	0.325
% 46	0.32794
% 47	0.33078
% 48	0.3337
% 49	0.33682
% 50	0.33978
% 51	0.34294
% 52	0.34608
% 53	0.34928
% 54	0.35248
% 55	0.35568
% 56	0.3589
% 57	0.36206
% 58	0.3655
% 59	0.3687
% 60	0.3719
% 61	0.37518
% 62	0.37858
% 63	0.38194
% 64	0.3853
% 65	0.3889
% 66	0.39242
% 67	0.39588
% 68	0.39942
% 69	0.403
% 70	0.4067
% 71	0.41036
% 72	0.414
% 73	0.4177
% 74	0.42142
% 75	0.4251
% 76	0.42898
% 77	0.43274
% 78	0.43664
% 79	0.4406
% 80	0.44448
% 81	0.44834
% 82	0.45226
% 83	0.45616
% 84	0.46014
% 85	0.46416
% 86	0.46818
% 87	0.47214
% 88	0.47618
% 89	0.48028
% 90	0.48424
% 91	0.48816
% 92	0.49214
% 93	0.4963
% 94	0.50026
% 95	0.50426
% 96	0.50832
% 97	0.51246
% 98	0.5165
% 99	0.5206
% 100	0.52464

==> csvs/ratio_OursSSR.tex <==
epochs Ratio
250	0.5209423602
251	0.5214820206
252	0.5220427811
253	0.5225839913
254	0.5230900347
255	0.5236263275
256	0.5241577327
257	0.5247202218
258	0.5252308249
259	0.5257631838
260	0.5262982547
261	0.5268366933
262	0.5273677409
263	0.527921468
264	0.5284378231
265	0.5289803743
266	0.5295231342
267	0.5300514996
268	0.530593276
269	0.5311289728
270	0.5316794515
271	0.5322214067
272	0.532743454
273	0.5332780778
274	0.5338168442
275	0.5343647003
276	0.5348894298
277	0.5354229212
278	0.5359712243
279	0.5365142524
280	0.5370539725
281	0.5376222432
282	0.5381286442
283	0.5386479199
284	0.5392012
285	0.539737314
286	0.5402569473
287	0.5407879055
288	0.5413438082
289	0.5418788493
290	0.542403996
291	0.5429446697
292	0.5434935093
293	0.5440141261
294	0.5445756912
295	0.5450878739
296	0.5456287265
297	0.5461640358
298	0.5467035472
299	0.5472439826

==> csvs/ratio_dm.tex <==
epochs	Ratio
251	0.6577
252	0.65746
253	0.65686
254	0.65606
255	0.65696
256	0.65682
257	0.65706
258	0.65708
259	0.65842
260	0.65668
261	0.65734
262	0.657
263	0.65722
264	0.65824
265	0.65598
266	0.65706
267	0.65692
268	0.6584
269	0.6573
270	0.6562
271	0.65624
272	0.65892
273	0.65752
274	0.65732
275	0.65706
276	0.65714
277	0.6569
278	0.65562
279	0.6569
280	0.65734
281	0.65768
282	0.6564
283	0.65808
284	0.65672
285	0.65688
286	0.65682
287	0.6588
288	0.6571
289	0.6566
290	0.65792
291	0.65726
292	0.65696
293	0.65714
294	0.65794
295	0.6569
296	0.65712
297	0.65632
298	0.65736
299	0.65664
300	0.65812

% epochs Ratio
% 30	0.76832
% 31	0.64214
% 32	0.66134
% 33	0.6511
% 34	0.64064
% 35	0.6441
% 36	0.65152
% 37	0.64854
% 38	0.65962
% 39	0.65178
% 40	0.6598
% 41	0.65618
% 42	0.66224
% 43	0.65376
% 44	0.66112
% 45	0.65592
% 46	0.66024
% 47	0.66484
% 48	0.66222
% 49	0.66348
% 50	0.65302
% 51	0.66206
% 52	0.6619
% 53	0.66598
% 54	0.6663
% 55	0.66682
% 56	0.66522
% 57	0.66426
% 58	0.66426
% 59	0.66562
% 60	0.66518
% 61	0.66496
% 62	0.66734
% 63	0.6649
% 64	0.65796
% 65	0.66944
% 66	0.66438
% 67	0.6676
% 68	0.66124
% 69	0.66866
% 70	0.65216
% 71	0.6646
% 72	0.65598
% 73	0.65928
% 74	0.6669
% 75	0.66538
% 76	0.65864
% 77	0.65906
% 78	0.65896
% 79	0.65768
% 80	0.65262
% 81	0.66158
% 82	0.65366
% 83	0.66028
% 84	0.66154
% 85	0.6544
% 86	0.66216
% 87	0.6544
% 88	0.6608
% 89	0.66386
% 90	0.6313
% 91	0.65902
% 92	0.66356
% 93	0.65498
% 94	0.65674
% 95	0.65256
% 96	0.65616
% 97	0.65468
% 98	0.65298
% 99	0.66082
% 100	0.65364
% 101	0.64982
% 102	0.65228
% 103	0.6521
% 104	0.65408
% 105	0.65254
% 106	0.65234
% 107	0.6505
% 108	0.6524
% 109	0.65036
% 110	0.65644
% 111	0.65306
% 112	0.65424
% 113	0.65626
% 114	0.65562
% 115	0.65268
% 116	0.65288
% 117	0.65592
% 118	0.6542
% 119	0.64964
% 120	0.65066
% 121	0.65834
% 122	0.6555
% 123	0.66306
% 124	0.65082
% 125	0.65618
% 126	0.65098
% 127	0.65276
% 128	0.65556
% 129	0.65288
% 130	0.65092
% 131	0.65428
% 132	0.65844
% 133	0.65254
% 134	0.65232
% 135	0.65642
% 136	0.65352
% 137	0.65518
% 138	0.6543
% 139	0.65106
% 140	0.65184
% 141	0.6549
% 142	0.64768
% 143	0.65162
% 144	0.65294
% 145	0.64806
% 146	0.65076
% 147	0.6525
% 148	0.6525
% 149	0.65324
% 150	0.65978
% 151	0.6571
% 152	0.65834
% 153	0.65866
% 154	0.65764
% 155	0.65964
% 156	0.65916
% 157	0.6596
% 158	0.6587
% 159	0.65818
% 160	0.65766
% 161	0.65948
% 162	0.65978
% 163	0.65834
% 164	0.6599
% 165	0.65772
% 166	0.6604
% 167	0.65982
% 168	0.65828
% 169	0.66004
% 170	0.65744
% 171	0.65848
% 172	0.65988
% 173	0.65878
% 174	0.65636
% 175	0.65708
% 176	0.65716
% 177	0.6572
% 178	0.65806
% 179	0.6581
% 180	0.6588
% 181	0.65854
% 182	0.65816
% 183	0.65774
% 184	0.65672
% 185	0.65598
% 186	0.65818
% 187	0.6578
% 188	0.65838
% 189	0.65576
% 190	0.65766
% 191	0.65774
% 192	0.65848
% 193	0.65824
% 194	0.6577
% 195	0.65698
% 196	0.6562
% 197	0.65718
% 198	0.65596
% 199	0.65772
% 200	0.65656
% 201	0.65726
% 202	0.65798
% 203	0.65646
% 204	0.65778
% 205	0.65712
% 206	0.6562
% 207	0.65624
% 208	0.65546
% 209	0.65686
% 210	0.6576
% 211	0.65712
% 212	0.65744
% 213	0.65794
% 214	0.6561
% 215	0.6576
% 216	0.65676
% 217	0.65838
% 218	0.65648
% 219	0.65716
% 220	0.6579
% 221	0.65716
% 222	0.65752
% 223	0.65572
% 224	0.65664
% 225	0.6556
% 226	0.65664
% 227	0.65636
% 228	0.6579
% 229	0.6571
% 230	0.65538
% 231	0.6553
% 232	0.65588
% 233	0.6566
% 234	0.65636
% 235	0.65612
% 236	0.6579
% 237	0.65732
% 238	0.657
% 239	0.65656
% 240	0.65696
% 241	0.65622
% 242	0.6558
% 243	0.65684
% 244	0.6561
% 245	0.65718
% 246	0.65746
% 247	0.6563
% 248	0.65588
% 249	0.6571
% 250	0.65732
% 251	0.6577
% 252	0.65746
% 253	0.65686
% 254	0.65606
% 255	0.65696
% 256	0.65682
% 257	0.65706
% 258	0.65708
% 259	0.65842
% 260	0.65668
% 261	0.65734
% 262	0.657
% 263	0.65722
% 264	0.65824
% 265	0.65598
% 266	0.65706
% 267	0.65692
% 268	0.6584
% 269	0.6573
% 270	0.6562
% 271	0.65624
% 272	0.65892
% 273	0.65752
% 274	0.65732
% 275	0.65706
% 276	0.65714
% 277	0.6569
% 278	0.65562
% 279	0.6569
% 280	0.65734
% 281	0.65768
% 282	0.6564
% 283	0.65808
% 284	0.65672
% 285	0.65688
% 286	0.65682
% 287	0.6588
% 288	0.6571
% 289	0.6566
% 290	0.65792
% 291	0.65726
% 292	0.65696
% 293	0.65714
% 294	0.65794
% 295	0.6569
% 296	0.65712
% 297	0.65632
% 298	0.65736
% 299	0.65664
% 300	0.65812

==> csvs/ratio_ssr.tex <==
epochs Ratio
250	0.56508
251	0.55924
252	0.57586
253	0.56194
254	0.56574
255	0.56456
256	0.58026
257	0.58382
258	0.5653
259	0.57352
260	0.58584
261	0.57314
262	0.5844
263	0.5678
264	0.59384
265	0.57318
266	0.57264
267	0.5874
268	0.58634
269	0.59616
270	0.57162
271	0.55868
272	0.56488
273	0.57072
274	0.57756
275	0.5817
276	0.57674
277	0.56838
278	0.59162
279	0.57288
280	0.60146
281	0.58926
282	0.59876
283	0.60234
284	0.58896
285	0.58972
286	0.61714
287	0.6043
288	0.59214
289	0.60412
290	0.5887
291	0.59072
292	0.60028
293	0.59594
294	0.60354
295	0.5932
296	0.608
297	0.59792
298	0.62206
299	0.60542

==> csvs/redmini_table.tex <==
% begin{table}[t]
%     \centering
%     \caption{Test accuracy \% (left table) and noise rate estimation \(\epsilon\) (right table) on CIFAR100~\citep{krizhevsky2009learning} under different IDN~\citep{xiao2015learning}. Other models results are presented in~\citep{garg2023instance,cheng2022instance}. Here, we use DivideMix~\citep{li2020dividemix} and InstanceGM~\citep{garg2023instance} as the baselines for our proposed work.}
%     \label{table:cifar100}
%     \begin{minipage}{.5\linewidth}
%         \centering
%          \begin{tabular}{l l l l l}
%     \toprule
%     \multirow{2}{*}{\bfseries Method } & \multicolumn{4}{c}{\bfseries Noise Rates - IDN} \\
%     \cmidrule{2 - 5} 
%     & \textbf{0.2} & \textbf{0.3} & \textbf{0.4} & \textbf{0.5} \\
%     \midrule
%     CE~\cite{yao2021instance} & 30.42 & 24.15 & 21.45 & 14.42 \\
%     PartT~\cite{xia2020part} & 65.33 & 64.56 & 59.73 & 56.80\\
%     kMEIDTM~\cite{cheng2022instance} & 69.16 & 66.76 & 63.46 & 59.18\\
%     \midrule
%     DivideMix~\cite{li2020dividemix} & 77.03 & 76.33 & 70.80 & 58.61\\
%     \rowcolor{Gray!25}\textbf{DivideMix-Ours} & \textbf{77.42} & \textbf{77.21} & \textbf{72.41} & \textbf{64.02}\\
%     % %\hdashline
%     % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.18}} & \scriptsize{\textbf{0.34}} & \scriptsize{\textbf{0.47}} & \scriptsize{\textbf{0.53}}\\
%     \midrule
%     InstanceGM~\cite{garg2023instance} & \textbf{79.69} & 79.21 & 78.47 & 77.19\\
%     \rowcolor{Gray!25} \textbf{InstanceGM-Ours} & 79.61 & \textbf{79.40} & \textbf{79.52} & \textbf{77.76}\\
%     % %\hdashline
%     % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.32}} & \scriptsize{\textbf{0.37}} & \scriptsize{\textbf{0.42}} & \scriptsize{\textbf{0.47}}\\
%     \bottomrule
%     \end{tabular}
%     \end{minipage}
%     \hspace{1.5cm}
%     \begin{minipage}{.35\linewidth}
%         \centering
%         \begin{tabular}{l l l}
%             \toprule
%             \multirow{2}{*}{\small{\bfseries Actual Noise}} & \multicolumn{2}{c}{\small{\bfseries Estimated} \(\epsilon\)} \\
%             \cmidrule{2 - 3} 
%             & \tiny{\textbf{DivideMix}} & \tiny{\textbf{InstanceGM}} \\
%             \midrule
%             \textbf{0.2} & 0.18 & 0.32\\
%             \textbf{0.3} & 0.34 & 0.37\\
%             \textbf{0.4} & 0.47 & 0.42\\
%             \textbf{0.5} & 0.53 & 0.47\\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}
% \end{table}
\begin{table}[t]
    \centering
    \caption{\emph{(left)} Test accuracy \% and \emph{(right)} final estimated noise rate \(\epsilon\) for red mini-ImageNet~\citep{jiang2020beyond}. Other methods' results are reported in~\citep{garg2023instance,xu2021faster}. We present the results with and without self-supervision~\citep{caron2021emerging}. We integrate DivideMix~\citep{li2020dividemix} and InstanceGM~\citep{garg2023instance} into our model, with the latter tested with and without self-supervision.}
    \label{table:redmini}
    \begin{subtable}[t]{.45\linewidth}
        \centering
        \addtolength{\tabcolsep}{-0.1em}
        \begin{tabular}{l c c c}
            \toprule
            \multirow{2}{*}{\bfseries Method} & \multicolumn{3}{c}{\bfseries Noise rate} \\
            \cmidrule{2-4}
             & \bfseries 0.4 & \bfseries 0.6 & \bfseries 0.8 \\
            \midrule
            CE~\cite{xu2021faster} &  42.70 & 37.30 & 29.76 \\
            MixUp~\cite{zhang2017mixup} &  46.40 & 40.58 & 33.58 \\
            MentorMix~\cite{jiang2020beyond} &  47.14 & 43.80 & 33.46 \\
            FaMUS~\cite{xu2021faster} & 51.42 &  45.10 & 35.50\\
            \midrule
            DivideMix~\cite{li2020dividemix} & 46.72 & 43.14 & 34.50 \\
            \rowcolor{Gray!25}\textbf{DivideMix-Ours} & \textbf{50.70} & \textbf{45.11} & \textbf{37.44} \\
            %\hdashline
            % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.39}} & 
            \midrule
            InstanceGM~\cite{garg2023instance} &  52.24 & 47.96 & 39.62 \\
            \rowcolor{Gray!25}\textbf{InstanceGM-Ours} &  \textbf{56.61} & \textbf{51.40} & \textbf{43.83} \\
            %\hdashline
            % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.38}} & \scriptsize{\textbf{0.55}} & \scriptsize{\textbf{0.74}} \\
            \midrule
            \midrule
            \multicolumn{4}{l}{\bfseries With self-supervised learning}\\
            \midrule
            % DivideMix~\cite{} & & & &  \\
            PropMix~\cite{cordeiro2021propmix} & 56.22 & 52.84 & 43.42\\
            \midrule
            InstanceGM-SS~\cite{garg2023instance} & 56.37 & 53.21 & 44.03\\
            \rowcolor{Gray!25}\textbf{InstanceGM-SS-Ours} & \textbf{58.29} & \textbf{53.60} & \textbf{45.47}\\
            %\hdashline
            % \rowcolor{Gray!10}\scriptsize{\textbf{Noise Rate} (\(\epsilon\))} & \scriptsize{\textbf{0.48}} & \scriptsize{\textbf{0.53}} & \scriptsize{\textbf{0.69}} \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{.5\linewidth}
        \centering
        \begin{tabular}{l c c c}
            \toprule
            \multicolumn{4}{l}{\bfseries Estimated noise rates} \\
            \midrule
            \multirow{2}{*}{\bfseries Method} & \multicolumn{3}{c}{\bfseries Actual noise rate} \\
            \cmidrule{2-4}
            & \bfseries 0.4 & \bfseries 0.6 & \bfseries 0.8 \\
            \midrule
            DivideMix & 0.39 & 0.58 & 0.73 \\
            InstanceGM & 0.38 & 0.55 & 0.74 \\
            InstanceGM-SS & 0.48 & 0.53 & 0.69 \\
            % \multirow{2}{*}{\bfseries \shortstack{Actual\\Noise}} & \multicolumn{3}{c}{\bfseries Estimated noise rate} \\
            % \cmidrule{2 - 4} 
            % & \textbf{DivideMix} & \textbf{InstanceGM} & \textbf{InstanceGM}-SS \\
            % \midrule
            % 0.4 & 0.39 & 0.38 & 0.48\\
            % 0.6 & 0.58 & 0.55 & 0.53\\
            % 0.8 & 0.73 & 0.74 & 0.69\\
            \bottomrule
        \end{tabular}
    \end{subtable}
\end{table}


==> csvs/training_time.tex <==
\begingroup
\begin{table}[htbp!]
        \caption{This table shows the training time of the base model DivideMix~\cite{li2020dividemix} and our approach with DivideMix~\cite{li2020dividemix} at \(0.5\) IDN~\cite{xia2020part} on the mentioned computational settings~\cref{subsec:implementation}.}
        \label{table:computation}
        \centering
        \begin{tabular}{c c}
        \toprule
        \textbf{Model} & \textbf{Time (hrs)} \\
        \midrule
        DivideMix~\cite{li2020dividemix} & \(7.2\) \\
        DivideMix-Ours & \(12.1\) \\
        \bottomrule
        \end{tabular}
\end{table} 
\endgroup


==> images/Rt_graphs/cc.tex <==
epochs	Rt
30	0.7603369483
31	0.7555153816
32	0.7554439877
32	0.7586395683
34	0.7587101238
35	0.7608923531
36	0.7584033669
37	0.7587270573
38	0.7578083226
39	0.7578166858
40	0.7536635027
41	0.7607259736
42	0.760857709
43	0.7589545336
44	0.7582755205
45	0.7571484907
46	0.758383287
47	0.7582261028
48	0.7612012533
49	0.7590870456
50	0.7603369483
51	0.7555153816
52	0.7554439877
53	0.7586395683
54	0.7587101238
55	0.7608923531
56	0.7584033669
57	0.7587270573
58	0.7578083226
59	0.7578166858
60	0.7536635027
61	0.7607259736
62	0.760857709
63	0.7589545336
64	0.7582755205
65	0.7571484907
66	0.758383287
67	0.7582261028
68	0.7612012533
69	0.7590870456
70	0.7599202038
71	0.7596824836
72	0.7586193757
73	0.7607915853
74	0.7573829466
75	0.7614237818
76	0.7587758133
77	0.760649824
78	0.7589780219
79	0.7615004005
80	0.7589821871
81	0.7588229439
82	0.7613220488
83	0.7602374827
84	0.7604665083
85	0.7594813731
86	0.7598375243
87	0.7608186885
88	0.7610525843
89	0.7609963513
90	0.7605245103
91	0.7592500133
92	0.7580804253
93	0.7607361479
94	0.7603950193
95	0.7605088361
96	0.7610003218
97	0.7611138952
98	0.7634977519
99	0.7610996951
100	0.7606719853
101	0.7613738497
102	0.7608347529
103	0.762721521
104	0.7634601464
105	0.7625246189
106	0.7645938817
107	0.7610488501
108	0.7660831307
109	0.7631470974
110	0.7595312332
111	0.7642756841
112	0.7613852114
113	0.7628110334
114	0.7652698975
115	0.766028636
116	0.7629296289
117	0.7627626259
118	0.7616273867
119	0.7646573867
120	0.7644490793
121	0.7647872083
122	0.7662263872
123	0.7630569109
124	0.7573535708
125	0.7610787197
126	0.7647083611
127	0.7648886983
128	0.76439843
129	0.7631915037
130	0.7628964439
131	0.7643010985
132	0.7621426718
133	0.7670305535
134	0.7643238914
135	0.7645337216
136	0.7665093402
137	0.7635769684
138	0.7647672841
139	0.7670401474
140	0.7643603695
141	0.7661793058
142	0.7666266583
143	0.7648048196
144	0.7690192189
145	0.7634227403
146	0.7656176224
147	0.7626321515
148	0.7642195118
149	0.7659864109
150	0.7615707685
151	0.7660699762
152	0.7657221148
153	0.7666085656
154	0.7664496774
155	0.7666081335
156	0.7670685542
157	0.7667554668
158	0.7671208565
159	0.7659171743
160	0.7655141227
161	0.7655684834
162	0.7659177183
163	0.7665456661
164	0.7660374664
165	0.7668511713
166	0.7663567239
167	0.7670009062
168	0.7668593035
169	0.7659343415
170	0.7666645894
171	0.7664351462
172	0.7671792699
173	0.7652590563
174	0.7658331971
175	0.7672992573
176	0.766280542
177	0.7662319549
178	0.7667732892
179	0.7669847249
180	0.7671465996
181	0.7663499638
182	0.7668247277
183	0.7663599341
184	0.7673971574
185	0.7677720742
186	0.7674878961
187	0.7674353483
188	0.7666850621
189	0.7668693327
190	0.7661513704
191	0.7659209691
192	0.7669516912
193	0.7667664491
194	0.7667975
195	0.766881744
196	0.767809148
197	0.7668680117
198	0.7662334182
199	0.7682148676
200	0.7677085233
201	0.7665253376
202	0.7662524902
203	0.7666477371
204	0.7667473895
205	0.765560255
206	0.766821047
207	0.7660777185
208	0.7656282015
209	0.7664073269
210	0.7670691536
211	0.7665589452
212	0.7665563134
213	0.7665399268
214	0.7663524159
215	0.7656692272
216	0.766934023
217	0.7660212687
218	0.7671667242
219	0.767393295
220	0.7664701256
221	0.7655784973
222	0.7663406646
223	0.7669572692
224	0.7668637714
225	0.7669498329
226	0.7674469168
227	0.7669580119
228	0.7665798038
229	0.7670402533
230	0.7674819812
231	0.7675158284
232	0.7669384916
233	0.7662246289
234	0.7660483215
235	0.7674084392
236	0.7678168203
237	0.7663613023
238	0.7676437569
239	0.767321626
240	0.7659339666
241	0.765858948
242	0.7674870325
243	0.7668048564
244	0.7666268379
245	0.7674824161
246	0.7671679787
247	0.7670220147
248	0.7675570355
249	0.7666045104
250	0.7683511487
251	0.7667456557
252	0.7677048202
253	0.7674493015
254	0.7669909877
255	0.7657909793
256	0.7672535065
257	0.7655636421
258	0.7676145602
259	0.7666805142
260	0.7669269342
261	0.7662545577
262	0.7671528841
263	0.7672434347
264	0.7672327069
265	0.7672239524
266	0.7654795722
267	0.7671925028
268	0.7669165676
269	0.7661545999
270	0.76651994
271	0.7672169598
272	0.7674233298
273	0.7663774065
274	0.7676553572
275	0.7667169355
276	0.7678824677
277	0.7670529657
278	0.7679443663
279	0.7669395953
280	0.7668292284
281	0.7665631167
282	0.7679608094
283	0.7682697791
284	0.7673145143
285	0.7685723674
286	0.767068633
287	0.7670568
288	0.7664977749
289	0.7674801722
290	0.7678824677
291	0.7672705214
292	0.7670925526
293	0.768304348
294	0.7681192057
295	0.7686131381
296	0.7673471906
297	0.7690564164
298	0.7685077829
299	0.7689137631
300	0.7684243086

==> images/Rt_graphs/coteaching_10.tex <==
epochs	Rt
1	1
2	0.95
3	0.9
4	0.85
5	0.8
6	0.75
7	0.7
8	0.65
9	0.6
10	0.55
11	0.5
12	0.5
13	0.5
14	0.5
15	0.5
16	0.5
17	0.5
18	0.5
19	0.5
20	0.5
21	0.5
22	0.5
23	0.5
24	0.5
25	0.5
26	0.5
27	0.5
28	0.5
29	0.5
30	0.5
31	0.5
32	0.5
33	0.5
34	0.5
35	0.5
36	0.5
37	0.5
38	0.5
39	0.5
40	0.5
41	0.5
42	0.5
43	0.5
44	0.5
45	0.5
46	0.5
47	0.5
48	0.5
49	0.5
50	0.5
51	0.5
52	0.5
53	0.5
54	0.5
55	0.5
56	0.5
57	0.5
58	0.5
59	0.5
60	0.5
61	0.5
62	0.5
63	0.5
64	0.5
65	0.5
66	0.5
67	0.5
68	0.5
69	0.5
70	0.5
71	0.5
72	0.5
73	0.5
74	0.5
75	0.5
76	0.5
77	0.5
78	0.5
79	0.5
80	0.5
81	0.5
82	0.5
83	0.5
84	0.5
85	0.5
86	0.5
87	0.5
88	0.5
89	0.5
90	0.5
91	0.5
92	0.5
93	0.5
94	0.5
95	0.5
96	0.5
97	0.5
98	0.5
99	0.5
100	0.5
101	0.5
102	0.5
103	0.5
104	0.5
105	0.5
106	0.5
107	0.5
108	0.5
109	0.5
110	0.5
111	0.5
112	0.5
113	0.5
114	0.5
115	0.5
116	0.5
117	0.5
118	0.5
119	0.5
120	0.5
121	0.5
122	0.5
123	0.5
124	0.5
125	0.5
126	0.5
127	0.5
128	0.5
129	0.5
130	0.5
131	0.5
132	0.5
133	0.5
134	0.5
135	0.5
136	0.5
137	0.5
138	0.5
139	0.5
140	0.5
141	0.5
142	0.5
143	0.5
144	0.5
145	0.5
146	0.5
147	0.5
148	0.5
149	0.5
150	0.5
151	0.5
152	0.5
153	0.5
154	0.5
155	0.5
156	0.5
157	0.5
158	0.5
159	0.5
160	0.5
161	0.5
162	0.5
163	0.5
164	0.5
165	0.5
166	0.5
167	0.5
168	0.5
169	0.5
170	0.5
171	0.5
172	0.5
173	0.5
174	0.5
175	0.5
176	0.5
177	0.5
178	0.5
179	0.5
180	0.5
181	0.5
182	0.5
183	0.5
184	0.5
185	0.5
186	0.5
187	0.5
188	0.5
189	0.5
190	0.5
191	0.5
192	0.5
193	0.5
194	0.5
195	0.5
196	0.5
197	0.5
198	0.5
199	0.5
200	0.5
201	0.5
202	0.5
203	0.5
204	0.5
205	0.5
206	0.5
207	0.5
208	0.5
209	0.5
210	0.5
211	0.5
212	0.5
213	0.5
214	0.5
215	0.5
216	0.5
217	0.5
218	0.5
219	0.5
220	0.5
221	0.5
222	0.5
223	0.5
224	0.5
225	0.5
226	0.5
227	0.5
228	0.5
229	0.5
230	0.5
231	0.5
232	0.5
233	0.5
234	0.5
235	0.5
236	0.5
237	0.5
238	0.5
239	0.5
240	0.5
241	0.5
242	0.5
243	0.5
244	0.5
245	0.5
246	0.5
247	0.5
248	0.5
249	0.5
250	0.5
251	0.5
252	0.5
253	0.5
254	0.5
255	0.5
256	0.5
257	0.5
258	0.5
259	0.5
260	0.5
261	0.5
262	0.5
263	0.5
264	0.5
265	0.5
266	0.5
267	0.5
268	0.5
269	0.5
270	0.5
271	0.5
272	0.5
273	0.5
274	0.5
275	0.5
276	0.5
277	0.5
278	0.5
279	0.5
280	0.5
281	0.5
282	0.5
283	0.5
284	0.5
285	0.5
286	0.5
287	0.5
288	0.5
289	0.5
290	0.5
291	0.5
292	0.5
293	0.5
294	0.5
295	0.5
296	0.5
297	0.5
298	0.5
299	0.5
300	0.5

==> images/Rt_graphs/coteaching_5.tex <==
epochs	Rt
1	1
2	0.9
3	0.8
4	0.7
5	0.6
6	0.5
7	0.5
8	0.5
9	0.5
10	0.5
11	0.5
12	0.5
13	0.5
14	0.5
15	0.5
16	0.5
17	0.5
18	0.5
19	0.5
20	0.5
21	0.5
22	0.5
23	0.5
24	0.5
25	0.5
26	0.5
27	0.5
28	0.5
29	0.5
30	0.5
31	0.5
32	0.5
33	0.5
34	0.5
35	0.5
36	0.5
37	0.5
38	0.5
39	0.5
40	0.5
41	0.5
42	0.5
43	0.5
44	0.5
45	0.5
46	0.5
47	0.5
48	0.5
49	0.5
50	0.5
51	0.5
52	0.5
53	0.5
54	0.5
55	0.5
56	0.5
57	0.5
58	0.5
59	0.5
60	0.5
61	0.5
62	0.5
63	0.5
64	0.5
65	0.5
66	0.5
67	0.5
68	0.5
69	0.5
70	0.5
71	0.5
72	0.5
73	0.5
74	0.5
75	0.5
76	0.5
77	0.5
78	0.5
79	0.5
80	0.5
81	0.5
82	0.5
83	0.5
84	0.5
85	0.5
86	0.5
87	0.5
88	0.5
89	0.5
90	0.5
91	0.5
92	0.5
93	0.5
94	0.5
95	0.5
96	0.5
97	0.5
98	0.5
99	0.5
100	0.5
101	0.5
102	0.5
103	0.5
104	0.5
105	0.5
106	0.5
107	0.5
108	0.5
109	0.5
110	0.5
111	0.5
112	0.5
113	0.5
114	0.5
115	0.5
116	0.5
117	0.5
118	0.5
119	0.5
120	0.5
121	0.5
122	0.5
123	0.5
124	0.5
125	0.5
126	0.5
127	0.5
128	0.5
129	0.5
130	0.5
131	0.5
132	0.5
133	0.5
134	0.5
135	0.5
136	0.5
137	0.5
138	0.5
139	0.5
140	0.5
141	0.5
142	0.5
143	0.5
144	0.5
145	0.5
146	0.5
147	0.5
148	0.5
149	0.5
150	0.5
151	0.5
152	0.5
153	0.5
154	0.5
155	0.5
156	0.5
157	0.5
158	0.5
159	0.5
160	0.5
161	0.5
162	0.5
163	0.5
164	0.5
165	0.5
166	0.5
167	0.5
168	0.5
169	0.5
170	0.5
171	0.5
172	0.5
173	0.5
174	0.5
175	0.5
176	0.5
177	0.5
178	0.5
179	0.5
180	0.5
181	0.5
182	0.5
183	0.5
184	0.5
185	0.5
186	0.5
187	0.5
188	0.5
189	0.5
190	0.5
191	0.5
192	0.5
193	0.5
194	0.5
195	0.5
196	0.5
197	0.5
198	0.5
199	0.5
200	0.5
201	0.5
202	0.5
203	0.5
204	0.5
205	0.5
206	0.5
207	0.5
208	0.5
209	0.5
210	0.5
211	0.5
212	0.5
213	0.5
214	0.5
215	0.5
216	0.5
217	0.5
218	0.5
219	0.5
220	0.5
221	0.5
222	0.5
223	0.5
224	0.5
225	0.5
226	0.5
227	0.5
228	0.5
229	0.5
230	0.5
231	0.5
232	0.5
233	0.5
234	0.5
235	0.5
236	0.5
237	0.5
238	0.5
239	0.5
240	0.5
241	0.5
242	0.5
243	0.5
244	0.5
245	0.5
246	0.5
247	0.5
248	0.5
249	0.5
250	0.5
251	0.5
252	0.5
253	0.5
254	0.5
255	0.5
256	0.5
257	0.5
258	0.5
259	0.5
260	0.5
261	0.5
262	0.5
263	0.5
264	0.5
265	0.5
266	0.5
267	0.5
268	0.5
269	0.5
270	0.5
271	0.5
272	0.5
273	0.5
274	0.5
275	0.5
276	0.5
277	0.5
278	0.5
279	0.5
280	0.5
281	0.5
282	0.5
283	0.5
284	0.5
285	0.5
286	0.5
287	0.5
288	0.5
289	0.5
290	0.5
291	0.5
292	0.5
293	0.5
294	0.5
295	0.5
296	0.5
297	0.5
298	0.5
299	0.5
300	0.5

==> images/Rt_graphs/ours.tex <==
epochs	Rt
20	0.3264611131
21	0.3268912733
22	0.3272133899
23	0.3275731885
24	0.3279156405
25	0.328237952
26	0.3285882002
27	0.3289222062
28	0.3292659575
29	0.3296264708
30	0.3299465734
31	0.3302988356
32	0.3306477195
33	0.3310029703
34	0.3313661474
35	0.3317124975
36	0.3320926315
37	0.3324659437
38	0.332878952
39	0.3333184677
40	0.3336982769
41	0.3341140139
42	0.3344983059
43	0.33493074
44	0.3353308845
45	0.3357538331
46	0.3361648923
47	0.3365671158
48	0.3369807088
49	0.3374744087
50	0.3378542829
51	0.3382954878
52	0.3387418252
53	0.3391736096
54	0.3395519894
55	0.339975068
56	0.3404062676
57	0.3408819062
58	0.341300047
59	0.3417491782
60	0.3421573138
61	0.3426639426
62	0.343030563
63	0.3434739119
64	0.3439577365
65	0.3443665218
66	0.3448222148
67	0.3452876532
68	0.3457278836
69	0.3461838365
70	0.346619584
71	0.3470995754
72	0.3475480568
73	0.347994979
74	0.3484578186
75	0.3489513236
76	0.3493424374
77	0.3498515999
78	0.350258891
79	0.3507442749
80	0.3511821663
81	0.3516266197
82	0.3521229184
83	0.3525995314
84	0.353009876
85	0.3534655041
86	0.3539424419
87	0.3544596606
88	0.3549071026
89	0.3553641599
90	0.3558405781
91	0.3563200498
92	0.3567576164
93	0.3572408563
94	0.3577197433
95	0.3581628972
96	0.3586360669
97	0.3591129398
98	0.3595937109
99	0.3601180762
100	0.3605691564
101	0.3610748106
102	0.3615517485
103	0.362029531
104	0.3625199175
105	0.3630579913
106	0.3635650748
107	0.3640949625
108	0.3645377266
109	0.3650285679
110	0.3655416286
111	0.3697359014
112	0.3665044701
113	0.367128433
114	0.367487582
115	0.3679908973
116	0.3685087007
117	0.3689828449
118	0.3694987643
119	0.3700312507
120	0.3704835004
121	0.3710066313
122	0.3715239799
123	0.3719802576
124	0.3725229442
125	0.3729996872
126	0.3734860456
127	0.3740167779
128	0.3744993681
129	0.3750479019
130	0.3756049466
131	0.3761680335
132	0.3766983759
133	0.3772571099
134	0.377859568
135	0.3783450168
136	0.3788590521
137	0.3794237632
138	0.3799081725
139	0.3804456615
140	0.381047405
141	0.3815140778
142	0.3820384431
143	0.3825719041
144	0.383103416
145	0.3836477268
146	0.3841967803
147	0.3847082168
148	0.3852629876
149	0.3857888472
150	0.3863177603
151	0.3868919569
152	0.387463035
153	0.3879245102
154	0.3884692109
155	0.3890236568
156	0.3895572478
157	0.3900756359
158	0.3906043541
159	0.3911416483
160	0.3916744596
161	0.3922075307
162	0.3927501523
163	0.393294853
164	0.3938246757
165	0.3943645686
166	0.394909659
167	0.3954439646
168	0.395993343
169	0.3965316767
170	0.3970724142
171	0.397597689
172	0.3981253678
173	0.3986717576
174	0.399258818
175	0.3997403038
176	0.4002919561
177	0.4008505601
178	0.4013656348
179	0.4018989658
180	0.4024825829
181	0.4030014259
182	0.4035421634
183	0.4040927762
184	0.4046962738
185	0.4051657403
186	0.4057012802
187	0.4062847674
188	0.4069249725
189	0.4073328483
190	0.4079332274
191	0.4084742898
192	0.4089920932
193	0.4094990468
194	0.4100494647
195	0.4105750644
196	0.4111252224
197	0.4116643357
198	0.4122101408
199	0.4127606237
200	0.4132992822
201	0.4138594455
202	0.4143889433
203	0.4149305904
204	0.4155228484
205	0.416025514
206	0.416592499
207	0.4171234262
208	0.4176937896
209	0.4182439476
210	0.4187867641
211	0.4193255526
212	0.4198711628
213	0.4204079372
214	0.4209714788
215	0.4215513277
216	0.4220531487
217	0.4223
218	0.4231874436
219	0.4237562478
220	0.4242374086
221	0.4247995859
222	0.4253380495
223	0.4258952242
224	0.4264322585
225	0.4271377575
226	0.4275324446
227	0.428083837
228	0.4287022775
229	0.4291984463
230	0.4297638071
231	0.4303011662
232	0.430830729
233	0.4315197909
234	0.4319480669
235	0.4325021881
236	0.4330552697
237	0.4335967869
238	0.4341876805
239	0.4347165936
240	0.4352610344
241	0.4358102828
242	0.4363681722
243	0.4368988395
244	0.4374645251
245	0.4380020142
246	0.4386441034
247	0.4391146094
248	0.4396622986
249	0.4402217472
250	0.4407650185
251	0.4413187498
252	0.44189574
253	0.4424247181
254	0.4430090499
255	0.443521136
256	0.4440978664
257	0.4446308726
258	0.4451793414
259	0.4457917398
260	0.4463157153
261	0.4468454081
262	0.4473981649
263	0.4479521561
264	0.4484997803
265	0.4491054219
266	0.4497115183
267	0.4501557767
268	0.450760054
269	0.4512987125
270	0.4518249619
271	0.4523915571
272	0.4529207951
273	0.4535097396
274	0.4540481383
275	0.454588421
276	0.4551272419
277	0.4557067335
278	0.4562608546
279	0.4567966869
280	0.4573485342
281	0.4579376411
282	0.4584733111
283	0.4590307781
284	0.459569729
285	0.4601252145
286	0.4607179922
287	0.461259152
288	0.4618066138
289	0.4623860079
290	0.4629092363
291	0.4634760588
292	0.4640220264
293	0.4645979771
294	0.4651307884
295	0.4657046276
296	0.4662319815
297	0.4668141693
298	0.4673552316
299	0.4679090604
300	0.4684666899

==> images/Rt_graphs/s2e.tex <==
epochs	Rt
1	1.022419867
2	0.9846309197
3	0.9539775841
4	0.928813935
5	0.9079155624
6	0.8903388482
7	0.8753742309
8	0.8624900627
9	0.8512849424
10	0.8414521668
11	0.8327542891
12	0.8250050665
13	0.818056596
14	0.8117900551
15	0.8061089577
16	0.8009341796
17	0.7962002433
18	0.7918525107
19	0.787845036
20	0.7841389073
21	0.7807009527
22	0.7775027201
23	0.7745196668
24	0.7717305108
25	0.7691167058
26	0.7666620149
27	0.7643521618
28	0.7621745427
29	0.760117988
30	0.7581725633
31	0.7563294029
32	0.7545805694
33	0.7529189349
34	0.75133808
35	0.7498322076
36	0.7483960687
37	0.7470248995
38	0.7457143655
39	0.7444605148
40	0.7432597359
41	0.7421087222
42	0.7410044399
43	0.7399441004
44	0.738925136
45	0.7379451784
46	0.7370020391
47	0.7360936932
48	0.7352182638
49	0.7343740088
50	0.7335593091
51	0.7327726576
52	0.7320126496
53	0.7312779746
54	0.7305674078
55	0.7298798038
56	0.7292140899
57	0.7285692603
58	0.7279443712
59	0.7273385358
60	0.7267509201
61	0.7261807391
62	0.7256272531
63	0.7250897644
64	0.7245676148
65	0.7240601819
66	0.7235668775
67	0.7230871452
68	0.7226204575
69	0.722166315
70	0.7217242438
71	0.7212937939
72	0.7208745381
73	0.7204660703
74	0.7200680043
75	0.7196799723
76	0.7193016243
77	0.7189326265
78	0.7185726609
79	0.7182214237
80	0.7178786254
81	0.7175439889
82	0.7172172497
83	0.7168981549
84	0.7165864623
85	0.7162819404
86	0.7159843672
87	0.71569353
88	0.7154092251
89	0.715131257
90	0.714859438
91	0.7145935881
92	0.7143335344
93	0.7140791106
94	0.7138301572
95	0.7135865204
96	0.7133480525
97	0.7131146114
98	0.7128860601
99	0.7126622668
100	0.7124431044
101	0.7122284506
102	0.7120181871
103	0.7118122003
104	0.7116103801
105	0.7114126206
106	0.7112188193
107	0.7110288774
108	0.7108426994
109	0.7106601928
110	0.7104812684
111	0.7103058399
112	0.7101338238
113	0.7099651392
114	0.7097997081
115	0.7096374545
116	0.7094783053
117	0.7093221894
118	0.7091690379
119	0.7090187841
120	0.7088713634
121	0.708726713
122	0.7085847721
123	0.7084454817
124	0.7083087844
125	0.7081746247
126	0.7080429486
127	0.7079137036
128	0.7077868389
129	0.7076623048
130	0.7075400534
131	0.7074200379
132	0.7073022128
133	0.707186534
134	0.7070729584
135	0.7069614443
136	0.7068519509
137	0.7067444386
138	0.7066388689
139	0.7065352043
140	0.7064334082
141	0.7063334449
142	0.7062352798
143	0.7061388792
144	0.70604421
145	0.7059512401
146	0.7058599384
147	0.7057702741
148	0.7056822177
149	0.70559574
150	0.7055108127
151	0.7054274082
152	0.7053454996
153	0.7052650605
154	0.7051860651
155	0.7051084885
156	0.7050323062
157	0.7049574941
158	0.704884029
159	0.7048118879
160	0.7047410486
161	0.7046714894
162	0.7046031888
163	0.704536126
164	0.7044702807
165	0.704405633
166	0.7043421634
167	0.7042798528
168	0.7042186827
169	0.7041586347
170	0.7040996911
171	0.7040418344
172	0.7039850475
173	0.7039293138
174	0.7038746168
175	0.7038209405
176	0.7037682692
177	0.7037165876
178	0.7036658807
179	0.7036161335
180	0.7035673319
181	0.7035194615
182	0.7034725085
183	0.7034264594
184	0.7033813007
185	0.7033370196
186	0.7032936031
187	0.7032510387
188	0.7032093142
189	0.7031684174
190	0.7031283365
191	0.7030890599
192	0.7030505763
193	0.7030128745
194	0.7029759435
195	0.7029397726
196	0.7029043511
197	0.7028696689
198	0.7028357156
199	0.7028024814
200	0.7027699565
201	0.7027381311
202	0.702706996
203	0.7026765417
204	0.7026467593
205	0.7026176397
206	0.7025891742
207	0.7025613542
208	0.7025341712
209	0.7025076168
210	0.702481683
211	0.7024563615
212	0.7024316446
213	0.7024075245
214	0.7023839935
215	0.7023610442
216	0.7023386691
217	0.7023168611
218	0.7022956129
219	0.7022749176
220	0.7022547683
221	0.7022351582
222	0.7022160806
223	0.702197529
224	0.7021794969
225	0.702161978
226	0.702144966
227	0.7021284548
228	0.7021124384
229	0.7020969108
230	0.7020818661
231	0.7020672986
232	0.7020532026
233	0.7020395725
234	0.7020264029
235	0.7020136883
236	0.7020014234
237	0.701989603
238	0.7019782219
239	0.701967275
240	0.7019567573
241	0.7019466639
242	0.7019369899
243	0.7019277306
244	0.7019188812
245	0.7019104372
246	0.7019023938
247	0.7018947467
248	0.7018874913
249	0.7018806234
250	0.7018741386
251	0.7018680326
252	0.7018623014
253	0.7018569407
254	0.7018519464
255	0.7018473147
256	0.7018430415
257	0.701839123
258	0.7018355552
259	0.7018323345
260	0.7018294571
261	0.7018269193
262	0.7018247175
263	0.7018228482
264	0.7018213077
265	0.7018200926
266	0.7018191996
267	0.7018186251
268	0.7018183659
269	0.7018184187
270	0.7018187802
271	0.7018194473
272	0.7018204167
273	0.7018216854
274	0.7018232503
275	0.7018251083
276	0.7018272564
277	0.7018296918
278	0.7018324114
279	0.7018354124
280	0.701838692
281	0.7018422473
282	0.7018460756
283	0.7018501742
284	0.7018545404
285	0.7018591714
286	0.7018640648
287	0.7018692178
288	0.7018746279
289	0.7018802926
290	0.7018862094
291	0.7018923759
292	0.7018987895
293	0.7019054479
294	0.7019123488
295	0.7019194897
296	0.7019268683
297	0.7019344825
298	0.7019423298
299	0.7019504082

==> images/Rt_graphs/ssr.tex <==
epochs	Rt
0	0.0010365546
1	0.0041586423
2	0.0060042749
3	0.0075922979
4	0.0105225701
5	0.0125448362
6	0.014005657
7	0.0163119276
8	0.0184195709
9	0.0215449036
10	0.0236081842
11	0.0255520405
12	0.0269232332
13	0.0301701171
14	0.032236654
15	0.0355317343
16	0.0364450871
17	0.0381502962
18	0.0413980126
19	0.0436433855
20	0.0466615714
21	0.0480639387
22	0.0501529178
23	0.0522201813
24	0.0542636611
25	0.056573348
26	0.0598588228
27	0.0613284004
28	0.0642681075
29	0.0668152502
30	0.0686830383
31	0.0713303231
32	0.0728136194
33	0.075469424
34	0.0778125959
35	0.0784113286
36	0.0815660759
37	0.0831995553
38	0.0861353234
39	0.0883263111
40	0.0914676361
41	0.0920724993
42	0.0951375285
43	0.0965480286
44	0.0994038431
45	0.1025673988
46	0.1042316851
47	0.1071028344
48	0.1081824317
49	0.1115423716
50	0.1121551927
51	0.115316273
52	0.1164772624
53	0.1191081327
54	0.1212965055
55	0.1240871838
56	0.1271112712
57	0.1283703121
58	0.131029672
59	0.1322645973
60	0.1343194304
61	0.1365162816
62	0.1387579396
63	0.1417808502
64	0.1450390892
65	0.1460487629
66	0.1487267246
67	0.1502707685
68	0.1527257068
69	0.1551057851
70	0.1567328171
71	0.1597349113
72	0.1615370682
73	0.1642192289
74	0.1674107333
75	0.1695491304
76	0.1719848101
77	0.1735589955
78	0.1759017633
79	0.178292784
80	0.1792703956
81	0.1822872046
82	0.1845637852
83	0.1860084343
84	0.1897538896
85	0.1908935126
86	0.1939087112
87	0.196089675
88	0.1984609563
89	0.2006592049
90	0.2026016084
91	0.2041104377
92	0.2058990378
93	0.2083452853
94	0.2109379009
95	0.2131193865
96	0.2151705491
97	0.2185642748
98	0.2193668723
99	0.2218764542
100	0.2238276494
101	0.2273151802
102	0.2292909028
103	0.2309274855
104	0.2327335102
105	0.2352078612
106	0.2375986594
107	0.2409909632
108	0.2417964526
109	0.243999317
110	0.2464803407
111	0.2496391426
112	0.2516667056
113	0.2541199372
114	0.2560563221
115	0.2590285162
116	0.2601522152
117	0.2622584421
118	0.2652945657
119	0.2669033701
120	0.2690899466
121	0.2727193957
122	0.274950712
123	0.275555782
124	0.2775058017
125	0.2814769223
126	0.2828593254
127	0.2853852007
128	0.2878101696
129	0.2901927778
130	0.2918083781
131	0.29379756
132	0.2955514139
133	0.2984197054
134	0.3009023462
135	0.3039304719
136	0.3055414201
137	0.3075001684
138	0.3094913568
139	0.3118843645
140	0.3147829006
141	0.3173189763
142	0.3185258996
143	0.3214581918
144	0.3227248817
145	0.3263887647
146	0.3277056704
147	0.3303820084
148	0.3315633055
149	0.3337997863
150	0.3359930077
151	0.3389844481
152	0.340504996
153	0.3425285782
154	0.3447461428
155	0.3487353231
156	0.3498743556
157	0.3527655572
158	0.3535642957
159	0.356291428
160	0.359066064
161	0.3608468806
162	0.3644391017
163	0.3655571859
164	0.3680824312
165	0.3696260007
166	0.3727591979
167	0.3742814057
168	0.377317678
169	0.378421709
170	0.3812277561
171	0.3834338857
172	0.3858286005
173	0.3889927594
174	0.3900707618
175	0.3920018744
176	0.3943093343
177	0.3964734028
178	0.400144658
179	0.4010150367
180	0.4044348478
181	0.4065607324
182	0.4078741622
183	0.4103107803
184	0.4123475991
185	0.4158504202
186	0.4165007585
187	0.4202241155
188	0.4213368966
189	0.422891194
190	0.4265013601
191	0.428385618
192	0.4313602877
193	0.4327867661
194	0.4353963172
195	0.4369396986
196	0.4405300362
197	0.4424036312
198	0.4442769767
199	0.4468486171
200	0.4475041061
201	0.4507802002
202	0.4532556286
203	0.4548259895
204	0.4584293745
205	0.4596606625
206	0.4628293695
207	0.4651220825
208	0.4670666939
209	0.4694431131
210	0.4716562156
211	0.4739339815
212	0.476159518
213	0.477203304
214	0.4796906548
215	0.4829475046
216	0.4840585491
217	0.4857924064
218	0.4887463251
219	0.4916803822
220	0.4922473056
221	0.4963840795
222	0.4978804897
223	0.5002168481
224	0.5028887762
225	0.5044546634
226	0.5058031762
227	0.5089873343
228	0.5118458002
229	0.5137030202
230	0.5165310517
231	0.5188104302
232	0.5210163932
233	0.5228614891
234	0.5240775466
235	0.5259593648
236	0.5288525311
237	0.5303151304
238	0.5331139897
239	0.534985223
240	0.5379185393
241	0.5400206268
242	0.5426392013
243	0.5452754016
244	0.5461987605
245	0.5501118817
246	0.5521272585
247	0.5536369306
248	0.5558379315
249	0.5574176263
250	0.560870218
251	0.5622944515
252	0.5655217012
253	0.566839772
254	0.568456177
255	0.5721202129
256	0.5728027731
257	0.5756987648
258	0.5788364339
259	0.5801926442
260	0.582668931
261	0.5856522872
262	0.5880006867
263	0.5899577571
264	0.5916677826
265	0.5940142195
266	0.5956257659
267	0.5976308526
268	0.6008358858
269	0.602765076
270	0.6048906471
271	0.6071729789
272	0.6100710093
273	0.6124522356
274	0.6145811406
275	0.6157376304
276	0.6183901462
277	0.6217734962
278	0.6231567258
279	0.6258485755
280	0.6278365635
281	0.6288234642
282	0.63174248
283	0.6335604921
284	0.6358807151
285	0.6381690991
286	0.6406402063
287	0.6434031015
288	0.6449628066
289	0.6478224399
290	0.6506451743
291	0.6520615544
292	0.6538415716
293	0.6564077186
294	0.6578495833
295	0.6605227885
296	0.6628776706
297	0.6656131418
298	0.6678984533
299	0.6707301656

==> images/ablation_graph.tex <==
\begin{figure}[t]
    \centering
    \begin{adjustbox}{max width=0.5\textwidth}
        \input{images/graph_ablation}
    \end{adjustbox}
        \caption{Ablation graph showing the learning pattern of the noise rate parameter estimation under different initialisation values, i.e., \(\epsilon = 0.001\) (blue), \(\epsilon = 0.1\) (orange), \(\epsilon = 0.9\) (red), when trained on DivideMix-ours case at \(0.5\) IDN~\cite{xia2020part} on CIFAR100~\cite{krizhevsky2009learning} \gustavo{Arpit, Can you place the table on the right of Table 5 inside this graph, and place this new graph in Table 5, on the right?}. 
        }
        \label{fig:ablation_supp}
\end{figure}

==> images/plots/001.tex <==
epochs	e
31	0.0005445674
32	0.0237743133
33	0.0246035954
34	0.0263856845
35	0.0298461591
36	0.0315455296
37	0.0338186197
38	0.0358299675
39	0.0383743875
40	0.0392549446
41	0.0409198003
42	0.0442487644
43	0.0462672039
44	0.0473069377
45	0.0499165541
46	0.0517005346
47	0.052886931
48	0.056143649
49	0.0579145475
50	0.0592035894
51	0.0622205512
52	0.0635202076
53	0.0652999292
54	0.0669519916
55	0.0700187342
56	0.0710353934
57	0.0746636795
58	0.0758955157
59	0.0778765045
60	0.0802908216
61	0.0822382812
62	0.0838434822
63	0.0864379643
64	0.0871383126
65	0.0910415557
66	0.0923522055
67	0.0934794559
68	0.0961093872
69	0.0991041317
70	0.1001536008
71	0.1019257743
72	0.1037720327
73	0.1072079515
74	0.1092401086
75	0.1096738362
76	0.1114650079
77	0.1135815345
78	0.1173114201
79	0.1183345551
80	0.1199998352
81	0.1219486493
82	0.1250253098
83	0.1257735139
84	0.1281487782
85	0.1300065676
86	0.1320147401
87	0.1339201049
88	0.1359504402
89	0.1380037501
90	0.1395424621
91	0.1427504386
92	0.1435548938
93	0.1461027725
94	0.1493712583
95	0.1509387094
96	0.1516216113
97	0.1547963951
98	0.1556490743
99	0.1594546401
100	0.1610536997
101	0.1619330725
102	0.1639445586
103	0.1658609365
104	0.1699340815
105	0.1697558435
106	0.1728664594
107	0.1745723642
108	0.1772977615
109	0.177809221
110	0.1799164137
111	0.1818608664
112	0.1851227858
113	0.1870684979
114	0.1889981839
115	0.1902743136
116	0.1923551658
117	0.193561099
118	0.1957754774
119	0.1981630771
120	0.2009544277
121	0.2034468211
122	0.2039669221
123	0.2070577113
124	0.2091532912
125	0.2115199023
126	0.2125476915
127	0.2148527889
128	0.2160491406
129	0.2190054262
130	0.2210057707
131	0.2219199517
132	0.2245784457
133	0.2264038836
134	0.2273947041
135	0.2301643566
136	0.2317110637
137	0.2344843807
138	0.2366245249
139	0.2386986355
140	0.239581128
141	0.2418958725
142	0.2436394045
143	0.2456572068
144	0.2478017284
145	0.2497891698
146	0.2516779265
147	0.2536098428
148	0.2560028551
149	0.258959363
150	0.2595505228
151	0.2625068806
152	0.2641622975
153	0.2652012633
154	0.2680073311
155	0.2694910708
156	0.2724975817
157	0.2744695882
158	0.2748882791
159	0.2776902714
160	0.2805874969
161	0.2809114689
162	0.2830166229
163	0.2851604267
164	0.2879906369
165	0.2902251357
166	0.2919486985
167	0.2923890065
168	0.2963442234
169	0.2972553521
170	0.2991452268
171	0.3002635178
172	0.3026313351
173	0.3050991896
174	0.3063812614
175	0.3099330283
176	0.3118877357
177	0.3127467544
178	0.3143326127
179	0.3162219263
180	0.3182880925
181	0.3200663997
182	0.3234892689
183	0.3243607649
184	0.3258722693
185	0.3290817173
186	0.3303262675
187	0.3318790237
188	0.3347301129
189	0.3359460547
190	0.3389287691
191	0.3412676127
192	0.3424525179
193	0.3438464954
194	0.3466864634
195	0.3488716048
196	0.3503788131
197	0.3508822693
198	0.3541475921
199	0.3549232113
200	0.356937069
201	0.3592953646
202	0.3611594735
203	0.362545957
204	0.3636217759
205	0.3665862636
206	0.367751786
207	0.370673156
208	0.3716150398
209	0.3745804044
210	0.3611780172
211	0.3773307694
212	0.3794828403
213	0.3813313449
214	0.3834507837
215	0.3833939386
216	0.3870939509
217	0.3886276258
218	0.38932688
219	0.3916271302
220	0.394066608
221	0.3951641664
222	0.3971736861
223	0.3986552201
224	0.4006299966
225	0.4021199901
226	0.4042963169
227	0.4049672335
228	0.4084063039
229	0.4085287814
230	0.4107167475
231	0.413244507
232	0.4136498671
233	0.4164967737
234	0.4180113447
235	0.4199125342
236	0.4206037583
237	0.4229094097
238	0.4238706646
239	0.4261928762
240	0.4284731647
241	0.4291322766
242	0.4313966215
243	0.4324332522
244	0.4339751852
245	0.4362229469
246	0.4371940652
247	0.4390186115
248	0.4413074513
249	0.4438295232
250	0.4450710423
251	0.4458993087
252	0.4487018168
253	0.4496739169
254	0.4516343748
255	0.452577558
256	0.4538477953
257	0.4557499443
258	0.4578714898
259	0.4598070185
260	0.46059748
261	0.4627748091
262	0.4631268179
263	0.465069855
264	0.46643324
265	0.4696128129
266	0.470951412
267	0.4731453367
268	0.4734048367
269	0.4744680757
270	0.4771148536
271	0.479119612
272	0.4799765626
273	0.4807338677
274	0.4823705685
275	0.4842025493
276	0.4857429813
277	0.4877928754
278	0.4892663724
279	0.4916212675
280	0.4917039809
281	0.4935379361
282	0.4948226779
283	0.4965268131
284	0.498457047
285	0.4993819279
286	0.5006618241
287	0.5025052731
288	0.5032901506
289	0.5043863796
290	0.5055432423
291	0.5063074244
292	0.5084052647
293	0.5091176027
294	0.5104255184
295	0.5114144759
296	0.5141021336
297	0.5149095614
298	0.5156034052
299	0.5163367439
300	0.5187220156
301	0.5196234561
302	0.51962346
303	0.5196512091
304	0.5196763211
305	0.5196213467
306	0.5196435978
307	0.5196754823
308	0.5196326549
309	0.5196436789
310	0.5196437859
311	0.5196435809

==> images/plots/01.tex <==
epochs	e
31	0.0992267728
32	0.1176340455
33	0.1210430397
34	0.1214598066
35	0.1226551484
36	0.1257938569
37	0.1272346468
38	0.1290894067
39	0.1309773101
40	0.1315239439
41	0.133655939
42	0.1358324918
43	0.1363312271
44	0.1379756741
45	0.1411347176
46	0.1422980585
47	0.1430541698
48	0.1452022654
49	0.1461902258
50	0.1488913228
51	0.1501210601
52	0.1511371484
53	0.1529806969
54	0.1552272874
55	0.1559597526
56	0.1577667202
57	0.1609930409
58	0.1619893638
59	0.1635477639
60	0.1653973938
61	0.1676841849
62	0.1693020537
63	0.1704458898
64	0.1728173247
65	0.1742708835
66	0.1754820694
67	0.1767827945
68	0.178315166
69	0.1799971519
70	0.1817757997
71	0.1845183252
72	0.1854822373
73	0.1866507174
74	0.1883852764
75	0.189451453
76	0.1913607412
77	0.1939124852
78	0.1954721126
79	0.1974194547
80	0.1982303282
81	0.1996970973
82	0.2018222139
83	0.2042528938
84	0.2060441448
85	0.2082068676
86	0.2097355989
87	0.2112702802
88	0.2113589456
89	0.2131221774
90	0.2150006122
91	0.216262491
92	0.2188091265
93	0.2204395582
94	0.2217129695
95	0.2246632313
96	0.2253765266
97	0.2264109582
98	0.2291442574
99	0.2304605858
100	0.2319870386
101	0.2336043541
102	0.235144055
103	0.237371996
104	0.2392610875
105	0.2396363448
106	0.24295071
107	0.2431892996
108	0.246402729
109	0.2473007864
110	0.2484848725
111	0.2509457102
112	0.2513578307
113	0.2539103382
114	0.2552127926
115	0.2561580865
116	0.2582112884
117	0.2609472038
118	0.2622400005
119	0.264335106
120	0.2649194278
121	0.2678546696
122	0.2690111129
123	0.2700798336
124	0.2713661647
125	0.2743640479
126	0.2744206587
127	0.2761820841
128	0.2789115626
129	0.2807780471
130	0.2818263544
131	0.2830026956
132	0.2850022087
133	0.2862121429
134	0.2889818107
135	0.2899902772
136	0.2907920517
137	0.2930780791
138	0.2946348358
139	0.2972650815
140	0.2982513903
141	0.3000013568
142	0.3019872098
143	0.3022741072
144	0.3042318266
145	0.306707629
146	0.3083250606
147	0.3096957731
148	0.3112975359
149	0.3127702128
150	0.3149329637
151	0.3164078072
152	0.3169209319
153	0.3193595731
154	0.3212519107
155	0.3224143326
156	0.3234216203
157	0.327002777
158	0.3280629864
159	0.3291942955
160	0.3313164231
161	0.3331098713
162	0.3332307393
163	0.3349715246
164	0.3371169055
165	0.3387658173
166	0.3405266479
167	0.3420002605
168	0.3446996813
169	0.3453335792
170	0.3466478687
171	0.3495664706
172	0.3509829743
173	0.3510038086
174	0.3543064684
175	0.3552405959
176	0.3577363663
177	0.3582177305
178	0.3597739863
179	0.3608005604
180	0.3624905391
181	0.3637449979
182	0.3664478777
183	0.3676819483
184	0.3689854891
185	0.371499572
186	0.3727035951
187	0.3734271756
188	0.3764335665
189	0.3780713933
190	0.3798019633
191	0.3813699882
192	0.3821107149
193	0.3852480497
194	0.3867197917
195	0.3881110983
196	0.3895753475
197	0.3911972232
198	0.3928572667
199	0.3944879266
200	0.3946985859
201	0.39728294
202	0.3983614303
203	0.4005040026
204	0.4007105311
205	0.4030461419
206	0.4044226962
207	0.4051453846
208	0.4077990405
209	0.407917724
210	0.3992389063
211	0.4110501128
212	0.4123923796
213	0.413894287
214	0.4160590477
215	0.4168521925
216	0.418454416
217	0.4202588745
218	0.4213907763
219	0.4227509789
220	0.4247704567
221	0.427085912
222	0.4275462066
223	0.4290699307
224	0.4302770939
225	0.4328477441
226	0.4340890437
227	0.4361277
228	0.4364344373
229	0.4389794433
230	0.440245904
231	0.4406693743
232	0.4430497
233	0.4435869625
234	0.4460695831
235	0.4475367793
236	0.447406177
237	0.4505820609
238	0.4514303815
239	0.4523557824
240	0.4542846799
241	0.4555715088
242	0.4555634281
243	0.4586058885
244	0.4590766638
245	0.4616380862
246	0.4624167062
247	0.46425635
248	0.4647092691
249	0.4670371153
250	0.4672551081
251	0.4691223536
252	0.4706938931
253	0.4718661837
254	0.4733711837
255	0.4734684117
256	0.4756690469
257	0.4772857281
258	0.4793438863
259	0.4802992046
260	0.4800339558
261	0.4823844991
262	0.484149852
263	0.4857299679
264	0.4857081214
265	0.4884314851
266	0.4893335279
267	0.4900252672
268	0.4918265672
269	0.4937933694
270	0.4933154326
271	0.4950628937
272	0.4975607537
273	0.498943894
274	0.4997128883
275	0.4996539866
276	0.5023236178
277	0.5024319011
278	0.5041089732
279	0.5054275656
280	0.507215854
281	0.5089097547
282	0.5090836354
283	0.5106775813
284	0.51103045
285	0.5133971949
286	0.5143930706
287	0.5143922057
288	0.5158008504
289	0.5163815124
290	0.5191329538
291	0.5185800768
292	0.5204224948
293	0.5210778391
294	0.5216462454
295	0.5239537901
296	0.5255018327
297	0.5256089911
298	0.5262518417
299	0.5269473052
300	0.5290387662
301	0.5301926957
302	0.5301278091
303	0.5316484325
304	0.5318923562
305	0.5319462902
306	0.5318352449
307	0.5318326254
308	0.5319375245
309	0.5310394642
310	0.5319236424
311	0.5310349862

==> images/plots/09.tex <==
epochs	e
31	0.8992559274
32	0.884266589
33	0.881282106
34	0.8810852658
35	0.8792716141
36	0.8785788183
37	0.8763441435
38	0.8749896744
39	0.874159669
40	0.871303043
41	0.8698265237
42	0.8690666417
43	0.8677403663
44	0.8658241726
45	0.8635927235
46	0.8619527534
47	0.8605733504
48	0.8592750675
49	0.8589292546
50	0.8559978334
51	0.854985163
52	0.8550083054
53	0.8532849218
54	0.8509144305
55	0.849028151
56	0.8490340692
57	0.8461547835
58	0.8449115588
59	0.8437741781
60	0.8430256319
61	0.8405602423
62	0.8402345199
63	0.8377658956
64	0.8371674729
65	0.835670615
66	0.8340425064
67	0.8318843233
68	0.8300640594
69	0.8297514665
70	0.826827378
71	0.8267415561
72	0.8235734255
73	0.8224211197
74	0.8212590443
75	0.8208579914
76	0.8180543704
77	0.8174182194
78	0.815857171
79	0.8134980008
80	0.8127059396
81	0.8101683018
82	0.8099994196
83	0.8079411887
84	0.8065604625
85	0.8043823477
86	0.8037224223
87	0.8031374547
88	0.8014517033
89	0.7994429915
90	0.7974962003
91	0.7957333206
92	0.7945907095
93	0.7945753425
94	0.7911035711
95	0.7907626954
96	0.7885163269
97	0.7881018227
98	0.7860518187
99	0.7844508751
100	0.7823276197
101	0.7817260684
102	0.7793623352
103	0.7788547912
104	0.7761844475
105	0.7759803368
106	0.7739081288
107	0.7725120368
108	0.771889657
109	0.7706748766
110	0.7694306766
111	0.7677640702
112	0.7652935609
113	0.764513404
114	0.7623698857
115	0.7609384317
116	0.7597138412
117	0.7576659962
118	0.7574005856
119	0.7551655194
120	0.7546250551
121	0.7519117229
122	0.7503164348
123	0.7502165546
124	0.7470116274
125	0.7471453776
126	0.7447147094
127	0.7439201659
128	0.7424704237
129	0.7399265629
130	0.7388899456
131	0.7381005285
132	0.7358999978
133	0.7356582719
134	0.7332457784
135	0.7321724145
136	0.72999819
137	0.729446421
138	0.7277520407
139	0.7253396307
140	0.7238699041
141	0.7224874306
142	0.7224868278
143	0.7196929307
144	0.7194799953
145	0.7177042629
146	0.7164112312
147	0.7148078791
148	0.7138108013
149	0.7120763361
150	0.7098205034
151	0.7098934989
152	0.7084912731
153	0.7060334087
154	0.7050543121
155	0.7041039139
156	0.7008221755
157	0.7001709513
158	0.6984202461
159	0.6966924855
160	0.6956101581
161	0.6950421503
162	0.6934930883
163	0.6920956796
164	0.6898892582
165	0.6882803906
166	0.6864612825
167	0.686603711
168	0.6841719852
169	0.6831700843
170	0.6815019518
171	0.6807574088
172	0.6791013444
173	0.6778053616
174	0.6756388678
175	0.6754185419
176	0.6740047498
177	0.6716116542
178	0.6706239348
179	0.6680182087
180	0.6668230902
181	0.666521813
182	0.6637910219
183	0.6633234444
184	0.661636722
185	0.6601890031
186	0.6594885653
187	0.6583269019
188	0.6560453756
189	0.654768296
190	0.6528504914
191	0.6509036833
192	0.6493658452
193	0.6483739052
194	0.6467430961
195	0.645515142
196	0.6453081933
197	0.6440571791
198	0.641850289
199	0.6397533351
200	0.6397575064
201	0.638516399
202	0.6365864098
203	0.6342619586
204	0.6337966087
205	0.6323767079
206	0.6302917757
207	0.6290399634
208	0.6280897795
209	0.6271260963
210	0.6359112311
211	0.6241613864
212	0.6230342131
213	0.621498652
214	0.6197840915
215	0.6194109797
216	0.618592981
217	0.6156321638
218	0.6150341201
219	0.6131014045
220	0.6122486798
221	0.6113607994
222	0.610544676
223	0.6092748448
224	0.6081541414
225	0.6063852661
226	0.6044643305
227	0.6033122593
228	0.6022680188
229	0.6016744945
230	0.6008246918
231	0.5995980155
232	0.5972574358
233	0.5965453537
234	0.5958820132
235	0.5937264825
236	0.5928140707
237	0.5912958518
238	0.5900650894
239	0.5877557482
240	0.5872605435
241	0.585911292
242	0.5857715997
243	0.5831843259
244	0.5821932936
245	0.5802414766
246	0.5794432201
247	0.5795599573
248	0.5779410897
249	0.5755934355
250	0.5754363553
251	0.5740430392
252	0.5727141124
253	0.5705969792
254	0.5699778504
255	0.5699980565
256	0.5679063536
257	0.5674752456
258	0.5658090983
259	0.5635719987
260	0.5633211386
261	0.5620454328
262	0.561760962
263	0.5590737748
264	0.5581673374
265	0.5579710706
266	0.556644534
267	0.5552990188
268	0.5539665557
269	0.5528891277
270	0.5507033512
271	0.5496332462
272	0.5493197014
273	0.5475064919
274	0.54671169
275	0.5456039924
276	0.5450089367
277	0.5434584423
278	0.5436423887
279	0.5412866093
280	0.5413028752
281	0.540124409
282	0.5377727693
283	0.537950196
284	0.5368044768
285	0.536050329
286	0.5347805029
287	0.5332105049
288	0.5320884347
289	0.531587753
290	0.530046847
291	0.5291891249
292	0.5277179422
293	0.5283286036
294	0.5267536702
295	0.5261936386
296	0.5249221589
297	0.52313902
298	0.5226658371
299	0.5212519038
300	0.5209543087
301	0.5209322883
302	0.5208183561
303	0.5208325341
304	0.5210385341
305	0.5215355892
306	0.5201974622
307	0.5209846273
308	0.5208437241
309	0.5202864527
310	0.5200183635
311	0.5201673528

==> main/tables/ablation_table.tex <==
% \begin{table*}[ht]
%         \centering
%         \caption{\emph{(left)} Ablation results showing the test accuracy \% on CIFAR100~\cite{krizhevsky2009learning} at \(0.5\) IDN~\cite{xia2020part}. First, we display the results of base DivideMix~\cite{li2020dividemix}, followed by the ideal case (result in \textit{italics}), where we assume to know the correct \(\epsilon=50\%\) for the sample selection before training. In the third case, we incorporate a pre-trained DivideMix~\cite{li2020dividemix} into our model, whilst the next case shows our proposed model and  DivideMix~\cite{li2020dividemix} being trained together, but using DivideMix's~\cite{li2020dividemix} sample selection curriculum, not our estimated \(\epsilon\). The last row shows the results of our proposed complete model with DivideMix~\cite{li2020dividemix}. \emph{(right)} This table shows the training time of the base model DivideMix~\cite{li2020dividemix} and our approach with DivideMix~\cite{li2020dividemix} at \(0.5\) IDN~\cite{xia2020part} on the mentioned computational settings~\cref{subsec:implementation}. }
%         \label{tab:ablation_cifar}
%         % \resizebox{0.4\textwidth}{!} {
%         \begin{subtable}[t]{.45\linewidth}
%         \addtolength{\tabcolsep}{-0.1em}
%         \centering
%         \begin{tabular}{l c}
%             \toprule
%             \bfseries Models &  \bfseries Test Accuracy (\%) \\
%             \midrule
%             DivideMix & 58.61 \\
%             DivideMix with fix \(\epsilon\) (ideal case) & 64.44 \\
%             Proposed with pre-trained DivideMix &  52.31\\
%             Proposed with original DivideMix (no \(\epsilon\)) & 56.30\\
%             \rowcolor{Gray!25} \textbf{DivideMix-Ours} & \textbf{64.02} \\
%             \bottomrule
%         \end{tabular}
%         \end{subtable}
%         \hfill
%         \begin{subtable}[t]{.3\linewidth}
%         \centering
%         \addtolength{\tabcolsep}{-0.4em}
%         \begin{tabular}{c c}
%         \toprule
%         \textbf{Model} & \textbf{Time (hrs)} \\
%         \midrule
%         DivideMix~\cite{li2020dividemix} & \(7.2\) \\
%         DivideMix-Ours & \(13.1\) \\
%         \bottomrule
%         \end{tabular}
%         \end{subtable}        
% \end{table*}

% \begin{table}[htbp!]
%         \caption{This table shows the training time of the base model DivideMix~\cite{li2020dividemix} and our approach with DivideMix~\cite{li2020dividemix} at \(0.5\) IDN~\cite{xia2020part} on the mentioned computational settings~\cref{subsec:implementation}.}
%         \label{table:computation}
%         \centering
%         \begin{tabular}{c c}
%         \toprule
%         \textbf{Model} & \textbf{Time (hrs)} \\
%         \midrule
%         DivideMix~\cite{li2020dividemix} & \(7.2\) \\
%         DivideMix-Ours & \(12.1\) \\
%         \bottomrule
%         \end{tabular}
% \end{table}

\begin{table}[ht]
    \centering
    \caption{Ablation results on CIFAR100~\cite{krizhevsky2009learning} at \(0.3\) and \(0.5\) IDN~\cite{xia2020part}. We display accuracy results under different configurations and compare the training time of our approach against DivideMix~\cite{li2020dividemix}. For computational settings, refer to~\cref{subsec:implementation}.\arpit{added 0.3 IDN results in the table, mixed precision training time}}
    \label{tab:ablation_cifar}
    \scalebox{0.8}{
    \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{\bfseries Models} & \multicolumn{2}{c}{\bfseries Accuracy (\%)} \\
        \cmidrule(lr){2-3}
        & \bfseries 0.3 & \bfseries 0.5 \\
        \midrule
        DivideMix~\cite{li2020dividemix} & 76.33 & 58.61 \\
        DivideMix with fixed \(\epsilon\) (ideal case) & 78.14 & 64.44 \\
        Our method with pre-trained DivideMix & 75.01 & 52.31 \\
        Our method with original DivideMix (no \(\epsilon\)) & 76.20 & 56.30 \\
        \rowcolor{Gray!25} \textbf{DivideMix-Ours} & 77.21 & 64.02 \\
        \midrule
        \multicolumn{3}{l}{\bfseries Training Time (GPU-hours)} \\
        \midrule
        DivideMix~\cite{li2020dividemix} & \multicolumn{2}{c}{7.20} \\
        \rowcolor{Gray!25} \textbf{DivideMix-Ours} & \multicolumn{2}{c}{8.50}\\
        \rowcolor{Gray!25} \textbf{DivideMix-Ours (Mixed Precision )} & \multicolumn{2}{c}{6.10}\\ % Added row for mixed precision
        \bottomrule
    \end{tabular}
    }
\end{table}

% \begin{table}[t]
% \centering
% \caption{Ablation results on CIFAR100~\cite{krizhevsky2009learning} at 
% 0.3 and 0.5 IDN~\cite{xia2020part}. We display accuracy results under different configurations and compare the training time of our approach against DivideMix~\cite{li2020dividemix}. For computational settings, refer to~\cref{subsec:implementation}.}\label{tab:ablation_cifar}
%     \scalebox{0.8}{
%     \begin{tabular}{lcc}
%     \toprule
%     \multirow{2}{*}{\bfseries Models} & \multicolumn{2}{c}{\bfseries Accuracy (\%)} \
%     \cmidrule(lr){2-3}
%     & \bfseries 0.3 & \bfseries 0.5 \
%     \midrule
%     DivideMix & 76.33 & 58.61 \
%     DivideMix with fixed \(\epsilon\) (ideal case) & 78.14 & 64.44 \
%     Our method with pre-trained DivideMix & 75.01 & 52.31 \
%     Our method with original DivideMix (no \(\epsilon\)) & 76.20 & 56.30 \
%     \rowcolor{Gray!25} \textbf{DivideMix-Ours} & 77.21 & 64.02 \
%     \midrule
%     \multicolumn{3}{l}{\bfseries Training Time (GPU-hours)} \
%     \midrule
%     DivideMix~\cite{li2020dividemix} & \multicolumn{2}{c}{7.20} \
%     \rowcolor{Gray!25} \textbf{DivideMix-Ours} & \multicolumn{2}{c}{8.50}\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table}
    % \begin{tabular}{l c}
    %     \toprule
    %     \bfseries Models & \bfseries Accuracy (\%) \\
    %     \midrule
    %     DivideMix & 58.61 \\
    %     DivideMix with fix \(\epsilon\) (ideal case) & 64.44 \\
    %     Our method with pre-trained DivideMix & 52.31 \\
    %     Our method with original DivideMix (no \(\epsilon\)) & 56.30 \\
    %     \rowcolor{Gray!25} \textbf{DivideMix-Ours} & 64.02 \\
    %     \midrule
    %     \midrule
    %     \multicolumn{2}{l}{\bfseries Training Time (GPU-hours)} \\
    %     \midrule
    %     DivideMix~\cite{li2020dividemix} & 7.20 \\
    %     \rowcolor{Gray!25} \textbf{DivideMix-Ours} & 8.50\\
    %     \bottomrule
    % \end{tabular}

==> main/tables/training_time.tex <==
\begingroup
\begin{table}[htbp!]
        \caption{This table shows the training time of the base model DivideMix~\cite{li2020dividemix} and our approach with DivideMix~\cite{li2020dividemix} at \(0.5\) IDN~\cite{xia2020part} on the mentioned computational settings~\cref{subsec:implementation}.}
        \label{table:computation}
        \centering
        \begin{tabular}{c c}
        \toprule
        \textbf{Model} & \textbf{Time (hrs)} \\
        \midrule
        DivideMix~\cite{li2020dividemix} & \(7.2\) \\
        DivideMix-Ours & \(12.1\) \\
        \bottomrule
        \end{tabular}
\end{table} 
\endgroup

